Reusable Slotwise Mechanisms

Agents with the ability to comprehend and reason about the dynamics of objects would be expected to exhibit improved robustness and generalization in novel scenarios. However, achieving this capability necessitates not only an effective scene representation but also an understanding of the mechanisms governing interactions among object subsets. Recent studies have made significant progress in representing scenes using object slots. In this work, we introduce Reusable Slotwise Mechanisms, or RSM, a framework that models object dynamics by leveraging communication among slots along with a modular architecture capable of dynamically selecting reusable mechanisms for predicting the future states of each object slot. Crucially, RSM leverages the Central Contextual Information (CCI), enabling selected mechanisms to access the remaining slots through a bottleneck, effectively allowing for modeling of higher order and complex interactions that might require a sparse subset of objects. Experimental results demonstrate the superior performance of RSM compared to state-of-the-art methods across various future prediction and related downstream tasks, including Visual Question Answering and action planning. Furthermore, we showcase RSM's Out-of-Distribution generalization ability to handle scenes in intricate scenarios.

==> figures/ablation_main.tex <==
% \begin{figure*}%
% \centering
% \subfigure[][2D Shapes]{%
% \label{fig:ex3-a}%
% \includegraphics[width=0.195\linewidth]{figures/ablation/main/Shapes.pdf}
% }%
% \subfigure[][3D Cubes]{%
% \label{fig:ex3-a}%
% \includegraphics[width=0.195\linewidth]{figures/ablation/main/Cubes.pdf}
% }%
% \subfigure[][Breakout]{%
% \label{fig:ex3-a}%
% \includegraphics[width=0.195\linewidth]{figures/ablation/main/Breakout.pdf}
% }%
% \subfigure[][Pong]{%
% \label{fig:ex3-a}%
% \includegraphics[width=0.195\linewidth]{figures/ablation/main/Pong.pdf}
% }%
% \subfigure[][Balls]{%
% \label{fig:ex3-a}%
% \includegraphics[width=0.195\linewidth]{figures/ablation/main/Balls.pdf}
% }%
% \caption{\textbf{Ablation study.} Clarify the importance of the CCI in mechanisms selection}%
% \label{fig:random_mechanisms}%
% \end{figure*}


\begin{figure*}[t]%
\centering
\vspace*{-2mm}
\subfigure{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Shapes_iid.pdf}
}%
\subfigure{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Cubes_iid.pdf}
}%
\subfigure{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Breakout_iid.pdf}
}%
\subfigure{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Pong_iid.pdf}
}%
\subfigure{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Balls_iid.pdf}
}\\
\setcounter{subfigure}{0}
\subfigure[][2D Shapes]{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Shapes_ood.pdf}
}%
\subfigure[][3D Cubes]{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Cubes_ood.pdf}
}%
\subfigure[][Breakout]{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Breakout_ood.pdf}
}%
\subfigure[][Pong]{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Pong_ood.pdf}
}%
\subfigure[][Balls]{%
\label{fig:ex3-a}%
\includegraphics[width=0.195\linewidth]{figures/ablation/full_bars/Balls_ood.pdf}
}%
\caption{\textbf{Ablation studies} to clarify the importance of the CCI in mechanisms selection. The original design of RSM, which includes the usage of CCI in mechanism assignment in a sequential manner, demonstrates the strongest results in all environments compared to the ablations.}%
\label{fig:ab_full}%
\vspace*{-2mm}
\end{figure*}

==> figures/disentanglement_ability_reconstruction.tex <==
% \begin{figure}[t]
%   \centering
%   \begin{tabular}{*{8}{@{\hspace{1px}}c}}
%     Step & Target & Predicted & Slot 1 & Slot 2 & Slot 3 & Slot 4 & Slot 5 \\
%     RSM &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
%         \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} \\
%     MBRL &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx0_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx1_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx2_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx3_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx4_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} \\
%     NPS &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_4_test_Cubes_NPS.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot0_4_test_Cubes_NPS.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot1_4_test_Cubes_NPS.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot2_4_test_Cubes_NPS.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot3_4_test_Cubes_NPS.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot4_4_test_Cubes_NPS.pdf} \\
%   \end{tabular}
%   \caption{Comparison of the reconstructed object from output slots at step 5 in the 3D Cubes environment}
%   \label{fig:reconstruct_slots}
% \end{figure}




\begin{figure}[t]
  \centering
  \begin{tabular}{*{8}{@{\hspace{1px}}c}}
    Step & Target & Predicted & Slot 1 & Slot 2 & Slot 3 & Slot 4 & Slot 5 \\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
        \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} \\
    % RSM ab par &
    %     \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predictedx_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} \\
    MBRL &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx0_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx1_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx2_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx3_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_slotx4_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} \\
    NPS &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot0_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot1_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot2_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot3_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_slot4_4_test_Cubes_NPS.pdf} \\
  \end{tabular}
  \caption{Comparison of the decoded slots at step 5 in the 3D Cubes environment. RSM generates the most meaningful slots and frame reconstruction compared to other models with modular design}
  \label{fig:reconstruct_slots}
\end{figure}



==> figures/envs_samples.tex <==
\begin{figure}[t]%
\centering
\subfigure{%
\includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf}
\includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf}
}%
\subfigure{%
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf}
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf}
}%
\subfigure{%
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Pong/1_actual_4_test_Modular_medium_3_Pong_7_3_xrandom10.pdf}
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Pong/1_actual_5_test_Modular_medium_3_Pong_7_3_xrandom10.pdf}
}%
\subfigure{%
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Breakout/0_actual_6_test_Modular_medium_3_Breakout_7_2_xrandom10.pdf}
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Breakout/0_actual_7_test_Modular_medium_3_Breakout_7_2_xrandom10.pdf}
}%
\subfigure{%
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Balls/1_actual_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf}
\includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/Balls/1_actual_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf}
}\\%
\setcounter{subfigure}{0}
\subfigure[][Shapes]{%
\label{fig:es_a}%
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_4_OOD2_Modular_medium_5_Shapes_4_5_attn10.pdf}
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_5_OOD2_Modular_medium_5_Shapes_4_5_attn10.pdf}
}%
\subfigure[][Cubes]{%
\label{fig:es_b}%
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_3_OOD2_Modular_medium_5_Cubes_3_5_attn10.pdf}
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_4_OOD2_Modular_medium_5_Cubes_3_5_attn10.pdf}
}%
\subfigure[][Pong]{%
\label{fig:es_c}%
\includegraphics[height=0.04\textheight]{figures/OOD samples/1_actual_2_OOD2_GNN_3_Pong10.pdf}
\includegraphics[height=0.04\textheight]{figures/OOD samples/1_actual_3_OOD2_GNN_3_Pong10.pdf}
}%
\subfigure[][Breakout]{%
\label{fig:es_d}%
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_2_OOD1_Modular_3_Breakout_32_5_MLP_Ctxtrue10.pdf}
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_3_OOD1_Modular_3_Breakout_32_5_MLP_Ctxtrue10.pdf}
}%
\subfigure[][Balls]{%
\label{fig:es_e}%
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_2_OOD1_Modular_medium_3_Balls_31_5_attn10.pdf}
\includegraphics[height=0.04\textheight]{figures/OOD samples/0_actual_3_OOD1_Modular_medium_3_Balls_31_5_attn10.pdf}
}%

\caption{Examples of visual inputs used in the experiments. Each pair of images in either row shows two consecutive frames of an environment (five pairs in total per row). The top row illustrates the iid data, and the bottom row depicts the OOD data samples. Environment pairs from left to right: 
grid world (\ref{fig:es_a}, \ref{fig:es_b}), Atari games (\ref{fig:es_c}, \ref{fig:es_d}, and Physics simulation (\ref{fig:es_e}).}%
\label{fig:envs_samples}%
\end{figure}


==> figures/full_step_main.tex <==
% \begin{figure}
%   \centering
%   \begin{tabular}{*{12}{@{\hspace{1px}}c}}
%     Step= & 0 & 1 & 2 & 3 & 4 & 5\\
%     Action= & 5-R & 3-U & 2-L & 1-U & 5-D & - \\
%     GT &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     RSM &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     % Assignment &
%     % [0, 3, 3, 3, 3]
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
%     % Attention &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
%     Mech=1 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=2 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=3 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=4 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=5 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\

%   \end{tabular}
%   \caption{Observation of mechanisms assignment and mechanisms performance during 5 rolling out steps in 2D Shapes environment. GT stands for ground-truth images. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots.}
%   \label{fig:fullsteps_main}
% \end{figure}

\begin{figure}[t]
\centering
\begin{Overpic}[abs,unit=1mm,grid=false,tics=5]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5\\
    Action= & 5-R & 3-U & 2-L & 1-U & 5-D & - \\
    GT &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    % Assignment &
    % [0, 3, 3, 3, 3]
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    % Attention &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    Mech=1 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=2 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=3 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=4 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=5 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\

  \end{tabular}}%

% \put(0,0){\color{red}\linethickness{0.6mm} \polygon(12.1, 82)(12.1, 53)(31,53)(31,73)(22,73)(22,82)}  %step 0->1
% \put(0,0){\color{green}\linethickness{0.6mm} \polygon(50, 82)(50, 53)(69.15,53)(69.15,73)(59.5,73)(59.5,82)} %step 4->5
% \put(0,0){\color{cyan}\linethickness{0.6mm} \polygon(31.5, 82)(31.5, 53)(49.6,53)(49.6,73)(40.6,73)(40.6,82)} %step 2->3
\put(0,0){\color{green}\linethickness{0.6mm} \polygon(21.5, 82)(21.5, 53)(40.6,53)(40.6,73)(31.4,73)(31.4,82)} %step 2->3
\put(0,0){\color{red}\linethickness{0.6mm} \polygon(40.8, 82)(40.8, 53)(59.6,53)(59.6,73)(50,73)(50,82)} %step 2->3
\put(0,0){\color{cyan}\linethickness{0.6mm} \polygon(40.6, 41.9)(40.6, 32.4)(59.5, 32.4)(59.5,41.9)} %step 2->3
% \put(0,0){\color{magenta}\linethickness{0.6mm} \polygon(40.6, 10.75)(40.6, 1.2)(59.5, 1.2)(59.5, 10.75)} %step 2->3
\end{Overpic}
\caption{Observation of mechanisms assignment and mechanisms performance during 5 rolling out steps in 2D Shapes environment. GT stands for ground-truth images. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots. See text for analysis.}
\label{fig:fullsteps_main}
\end{figure}

==> figures/full_step_main_2.tex <==
% \begin{figure}
%   \centering
%   \begin{tabular}{*{12}{@{\hspace{1px}}c}}
%     Step= & 0 & 1 & 2 & 3 & 4 & 5\\
%     Action= & 5-R & 3-U & 2-L & 1-U & 5-D & - \\
%     GT &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     RSM &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     % Assignment &
%     % [0, 3, 3, 3, 3]
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
%     % Attention &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
%     % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
%     Mech=1 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=2 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=3 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=4 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
%     Mech=5 &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
%     \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\

%   \end{tabular}
%   \caption{Observation of mechanisms assignment and mechanisms performance during 5 rolling out steps in 2D Shapes environment. GT stands for ground-truth images. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots.}
%   \label{fig:fullsteps_main}
% \end{figure}

\begin{figure}[h]
\centering
\begin{Overpic}[abs,unit=1mm,grid=false,tics=5]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5\\
    Action= & 5-R & 3-U & 2-L & 1-U & 5-D & - \\
    Groundtruth &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Prediction &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Masking Case 1 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_1_2.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_2_2.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_3_2.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_4_2.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_5_2.pdf} \\
    Masking Case 2 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_1_1.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_2_1.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_3_1.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_4_1.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/cases/7_predictedx_5_1.pdf} \\
    
  \end{tabular}}%

% \put(0,0){\color{red}\linethickness{0.6mm} \polygon(12.1, 82)(12.1, 53)(31,53)(31,73)(22,73)(22,82)}  %step 0->1
% \put(0,0){\color{green}\linethickness{0.6mm} \polygon(50, 82)(50, 53)(69.15,53)(69.15,73)(59.5,73)(59.5,82)} %step 4->5
% \put(0,0){\color{cyan}\linethickness{0.6mm} \polygon(31.5, 82)(31.5, 53)(49.6,53)(49.6,73)(40.6,73)(40.6,82)} %step 2->3


% \put(0,0){\color{green}\linethickness{0.6mm} \polygon(21.5, 82)(21.5, 53)(40.6,53)(40.6,73)(31.4,73)(31.4,82)} %step 2->3
% \put(0,0){\color{red}\linethickness{0.6mm} \polygon(40.8, 82)(40.8, 53)(59.6,53)(59.6,73)(50,73)(50,82)} %step 2->3
% \put(0,0){\color{cyan}\linethickness{0.6mm} \polygon(40.6, 41.9)(40.6, 32.4)(59.5, 32.4)(59.5,41.9)} %step 2->3



% \put(0,0){\color{magenta}\linethickness{0.6mm} \polygon(40.6, 10.75)(40.6, 1.2)(59.5, 1.2)(59.5, 10.75)} %step 2->3
\end{Overpic}
\caption{Observation of mechanisms assignment and mechanisms performance during 5 rolling out steps in 2D Shapes environment. GT stands for ground-truth images. In \textit{Masking Cases}, we present reconstruction when the CCI is masked out in (1) the mechanism selection process, and (2) in the computation of state transitions. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots.}
\label{fig:fullsteps_main}
\end{figure}

==> figures/full_step_main_4.tex <==
\begin{figure}[h]
\centering
\begin{Overpic}[abs,unit=1mm,grid=false,tics=5]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5\\
    Action= & 5-R & 3-U & 2-L & 1-U & 5-D & - \\
    GT &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Attention Weight &
    \includegraphics[height=0.04\textheight]{figures/full_steps/attn/0.png} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/attn/1.png} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/attn/2.png} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/attn/3.png} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/attn/4.png} & -\\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
  \end{tabular}}%
\end{Overpic}
\caption{Attention weight visualization over 5 roll-out prediction steps. The visualization shows that RSM with the CCI can recognize the involved objects needed to predict changes of each slot.}
\label{fig:fullsteps_main}
\end{figure}

==> figures/full_steps.tex <==
\begin{figure}
  \centering
  \begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    Action= & 5-R & 3-U & 2-L & 1-U & 5-D & 3-R & 1-R & 4-L & 3-L & 3-D & - \\
    Groundtruth &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    % Assignment &
    % [0, 3, 3, 3, 3]
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    % Attention &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    Mech=1 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=2 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=3 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=4 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=5 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\

  \end{tabular}
  \caption{Observation of mechanisms assignment and mechanisms performance during 10 rolling out steps in 2D Shapes environment. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots. }
  \label{fig:fullsteps}
\end{figure}

==> figures/full_steps_2.tex <==
\begin{figure}
  \centering
  \begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    Action= & 5-R & 3-U & 2-L & 1-U & 5-D & 3-R & 1-R & 4-L & 3-L & 3-D & - \\
    Groundtruth &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    % Masked Case 1 &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    % Masked Case 2 &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    % Assignment &
    % [0, 3, 3, 3, 3]
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    % Attention &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    Mech=1 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_0_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=2 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_1_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=3 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_2_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=4 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_3_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\
    Mech=5 &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_actual_0_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_1_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_2_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_3_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_4_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_5_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_6_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_7_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_8_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_9_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/full_steps/7_predicted_4_10_test_Modular_5_Shapes_attn2_Ctxtrue10.pdf} \\

  \end{tabular}
  \caption{Observation of mechanisms assignment and mechanisms performance during 10 rolling out steps in 2D Shapes environment. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots. }
  \label{fig:fullsteps}
\end{figure}

==> figures/full_steps_balls.tex <==
\begin{figure}
  \centering
  \begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Step= & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    Groundtruth &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    \textbf{RSM} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    % Assignment &
    % [0, 3, 3, 3, 3]
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    % Attention &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_1_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_2_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_3_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_4_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_5_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_6_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_7_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_8_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_9_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} &
    % \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/IID/RSM/Balls/1_predictedx_10_test_Modular_medium_3_Ballsx_7_5_xrandom10.pdf} \\
    \textbf{Mech=1} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_1/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    \textbf{Mech=2} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_2/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    \textbf{Mech=3} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_3/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    \textbf{Mech=4} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_4/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    \textbf{Mech=5} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/origin/7_actual_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_predictedx_10_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 1 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx0_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 2 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx1_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\
    Slot 3 & &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_0_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_1_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_2_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_3_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_4_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_5_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_6_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_7_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_8_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.03\textheight]{figures/reconstructed_imgs/full_balls/mech_5/7_slotx2_9_test_Modular_3_Balls_4_5_attn2_Ctxtrue10.pdf} \\

  \end{tabular}
  \caption{Observation of mechanisms assignment and mechanisms performance during 10 rolling out steps in Balls  environment. The last 5 rows represent the reconstruction with a single mechanism assigned for all slots.}
  \label{fig:fullsteps_balls}
\end{figure}

==> figures/mechs.tex <==
\subsection{Number of Mechanisms} \label{ap:num_mech}

\begin{figure}%
\centering
\subfigure[][2D Shapes]{%
\label{fig:ex3-a}%
\includegraphics[width=0.6\linewidth]{figures/mechs/Shapes.pdf}
} \\
\subfigure[][3D Cubes]{%
\label{fig:ex3-b}%
\includegraphics[width=0.6\linewidth]{figures/mechs/Cubes.pdf}
}\\
\subfigure[][Breakout]{%
\label{fig:ex3-c}%
\includegraphics[width=0.6\linewidth]{figures/mechs/Breakout.pdf}
} \\%
\subfigure[][Pong]{%
\label{fig:ex3-d}%
\includegraphics[width=0.6\linewidth]{figures/mechs/Pong.pdf}
}\\%
\subfigure[][Balls]{%
\label{fig:ex3-d}%
\includegraphics[width=0.6\linewidth]{figures/mechs/Balls.pdf}
}\\%
\caption{Effects of number of mechanisms on H@1}%
\label{fig:num_mechs}%
\end{figure}


In this section, we discuss the effect of the number of mechanisms on different environments.
In Figure \ref{fig:num_mechs}, we illustrate the changes in H@1 performance when the number of mechanisms is 3, 5, and 7 sequentially.
We can observe an optimal number of mechanisms for each environment, which are $[5, 5, 5, 3, 7]$ in the order from top to bottom.
The performance drop in cases with less or more than the optimal number signals the requirement of redefining task complexity.
For instance, from the Appendix \ref{ap:mech_fulls} about Balls environment, we know that slots in Balls learn multiple circular trajectories.
Therefore, a large number of mechanisms should be used to promote the model to handle more cases of trajectory and improve performance.

==> figures/random_mechanisms.tex <==
\begin{figure*}%
\centering
\subfigure[][2D Shapes]{%
\label{fig:ex3-a}%
\includegraphics[width=0.19\linewidth]{figures/mechs/random_mechs/Shapes.pdf}
}%
\subfigure[][3D Cubes]{%
\label{fig:ex3-a}%
\includegraphics[width=0.19\linewidth]{figures/mechs/random_mechs/Cubes.pdf}
}%
\subfigure[][Breakout]{%
\label{fig:ex3-a}%
\includegraphics[width=0.19\linewidth]{figures/mechs/random_mechs/Breakout.pdf}
}%
\subfigure[][Pong]{%
\label{fig:ex3-a}%
\includegraphics[width=0.19\linewidth]{figures/mechs/random_mechs/Pong.pdf}
}%
\subfigure[][Balls]{%
\label{fig:ex3-a}%
\includegraphics[width=0.19\linewidth]{figures/mechs/random_mechs/Balls.pdf}
}%
\caption{\textbf{Input-based  one-hot mechanism selection is important for model performance.} To understand the contribution of mechanism selection to model performance in the visual task, RSM is compared with a modified version in which a random mechanism is assigned for the prediction at each time step. The results suggest that the mechanism picking learned by RSM has a significant contribution to performance on both in-distribution and out-of-distribution test sets. }%
\label{fig:random_mechanisms}%
\end{figure*}

==> figures/reconstruct_Cubes_main.tex <==
\begin{figure}
  \centering
  \begin{tabular}{*{11}{@{\hspace{1px}}c}}
    Step= & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
    GT &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    RSM (Ours) &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    GNN &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_0_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_1_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_2_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_3_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_4_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_5_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_6_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_7_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_8_test_GNN_medium_5_Cubes10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/GNN/0_predicted_9_test_GNN_medium_5_Cubes10.pdf} \\
    MBRL &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/0_predicted_0_test_Modular_medium_5_Cubes_-1_-1_xrandom10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_1_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_2_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_3_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_4_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_5_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_6_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_7_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_8_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/MBRL/Cubes/0_predicted_9_test_Modular_5_Cubes_-1_-1_MLP_Ctxfalse10.pdf} \\
    NPS &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_0_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_1_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_2_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_3_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_4_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_5_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_6_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_7_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_8_test_Cubes_NPS.pdf} &
    \includegraphics[height=0.05\textheight]{figures/reconstructed_imgs/IID/NPS/Cubes/0_predicted_9_test_Cubes_NPS.pdf} \\

    
    % \includegraphics[height=0.05\textheight]{example-image-a} \\
    
  \end{tabular}
  \caption{Reconstruction comparison on 3D Cubes dataset}
  \label{fig:reconstruct_cubes}
\end{figure}

==> figures/reconstruction.tex <==
% \begin{figure*}
% \subfigure{\includegraphics[height=0.04\textheight]{example-image}}
% \subfigure{\includegraphics[height=0.04\textheight]{example-image}}

% \caption{aaa}
% \end{figure*}


\begin{figure}
  \centering
  \begin{tabular}{*{8}{@{\hspace{1px}}c}}
    Step & Target & Predicted & Slot 1 & Slot 2 & Slot 3 & Slot 4 & Slot 5 \\
    1 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_0_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    2 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_1_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    3 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_2_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    4 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_3_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    5 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    6 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_5_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    7 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_6_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    8 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_7_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    9 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_8_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    10 &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_9_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} \\
    
  \end{tabular}
  \caption{Blah}
  \label{materialflowChart}
\end{figure}



==> figures/slots_cube_ap.tex <==
\begin{figure}[t]
  \centering
  \begin{tabular}{*{8}{@{\hspace{1px}}c}}
    Step & Target & Predicted & Slot 1 & Slot 2 & Slot 3 & Slot 4 & Slot 5 \\
    RSM &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/Target/0_actual_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
        \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_5_Cubes_4_5_attn2_Ctxtrue10.pdf} \\
    RSM ab par &
        \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predicted_4_test_Modular_medium_5_Cubes_7_5_xrandom10.pdf} &
    
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_predictedx_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot0_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot1_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot2_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot3_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} &
    \includegraphics[height=0.04\textheight]{figures/reconstructed_imgs/IID/RSM/0_slot4_4_test_Modular_5_Cubes_43_5_attn2_Ctxtrue10.pdf} \\
  \end{tabular}
  \caption{Comparison of the reconstructed slots at step 5 of the sequential and parallel version in the 3D Cubes environment. The parallel version misses the information visibility order due to the absence of information integration by the CCI in a sequential manner.}
  \label{fig:reconstruct_slots_par}
\end{figure}



==> sections/ap_1.tex <==
% \input{sections/pseudo_RSM.tex}

\section{End-to-end training strategy}
\subsection{Environments}
We demonstrate the effectiveness of RSM on five datasets from three categories: Atari games (Pong and Breakout), manipulation on a grid world (2D Shapes and 3D Cubes \cite{Kipf2020Contrastive}), and Physics simulation (Balls \cite{Kipf2020Contrastive}).
At each time step, given an action and a single frame in the case of the grid world datasets, or two consecutive frames in the case of Atari games and Balls, the task is to predict the next state after the action is performed.
We follow \cite{Kipf2020Contrastive, NEURIPS2021_10907813} to generate the in-distribution (iid) and OOD datasets for each environment, as described in Appendix \ref{ap:envs}.
In addition, Figure \ref{fig:envs_samples} visually compares the iid and OOD data.
\input{figures/envs_samples.tex}

\subsection{Baselines}
We pick C-SWM \cite{Kipf2020Contrastive} as the most promising candidate among GNN-based methods for modeling transition dynamics. C-SWM uses the same inputs as RSM but uses shared node and edge update functions for modeling all transitions and predisposes the connections among slots to be dense. On the other hand, \cite{BENCHMARKS2021_8f121ce0} propose an RL benchmark for evaluating structure learning and uses modular architecture where each slot can be updated by any of a given set of mechanisms; however, mechanisms take as input all other slots, i.e., dense connectivity is a feature of this method too. We refer to it as MBRL \cite{BENCHMARKS2021_8f121ce0}. Finally, NPS from \cite{goyal2021neural} is the closest to our approach that has a set of reusable mechanisms used with slot representations, but compared to others, assumes all interactions to be pairwise, and thus, results in very sparse communications in contrast to the flexibility of RSM in that regard.

\subsection{Experimental and Analytical Results}
\input{tables/ood_main}
\subsubsection{Next State Prediction}
% Table \ref{tab:merge_table} summarizes the comparison of the quantitative results between the proposed method and baselines on iid and OOD test sets.
% Overall, RSM achieves the highest scores in both iid and OOD settings in most of the cases and environments, which supports the hypothesis of improved generalization and robustness when learning the communication of slots in the latent space.
% We find that the baselines that do not use a modularized design for modeling the dynamics, such as C-SWM \cite{Kipf2020Contrastive}, or do not utilize the general contextual information, such as \cite{BENCHMARKS2021_8f121ce0,goyal2021neural}, show a significant drop in OOD performance, especially in the Atari games and Physics simulation environments.
% RSM yields a smaller gap between the iid and OOD results and remains the most stable method for predicting 10 steps into the future in both iid and OOD setups
% The main reason for this gap may be attributed to the sequential communication of slots through the attention bottleneck of the CCI within each prediction step.
% More specifically, the CCI in RSM facilitates the effectiveness of communications among slots by making it easier for a slot to observe the changes of others before predicting its update. This would reduce the small prediction errors from each slot that accumulate and corrupt the prediction (see the analysis in Section \ref{ap:ab}).
% Consequently, all of the baselines that do not allow observing the changes of other slots fare poorly on 10-step rolling-out predictions.

Table \ref{tab:merge_table} summarizes the quantitative results of the proposed method and baselines on both iid and OOD test sets. In most cases and environments, RSM consistently outperforms the other models, supporting the hypothesis that learning the communication of slots in the latent space enhances generalization and robustness. The models that do not use a modularized design for modeling dynamics, such as C-SWM \cite{Kipf2020Contrastive}, or fail to utilize general contextual information, such as \cite{BENCHMARKS2021_8f121ce0,goyal2021neural}, exhibit significant drops in OOD performance, particularly in the Atari games and Physics simulation environments. Furthermore, RSM yields a smaller gap between the iid and OOD results and remains the most stable method for predicting 10 steps into the future in both iid and OOD setups.

The primary reason for this gap is the sequential communication of slots through the attention bottleneck of the CCI within each prediction step. In particular, the CCI in RSM improves the effectiveness of communications among slots by making it easier for a slot to observe changes in others before predicting its update. This reduces the small prediction errors from each slot that accumulate and corrupt the prediction, as demonstrated in the analysis presented in Section \ref{ap:ab}. Consequently, all baselines that do not allow observing changes in other slots perform poorly in 10-step rolling-out predictions.


% -------------
\subsubsection{Mechanisms are not interchangeable, and a proper assignment is necessary}

\input{figures/random_mechanisms.tex}
Figure \ref{fig:random_mechanisms} supports our hypothesis that mechanisms tend to specialize in modeling non-overlapping transitions. We can see that if we ignore our mechanism selection procedure and assign a mechanism to each slot at random, the performance drops significantly as the rollout continues further in time, supporting the hypothesis that mechanisms are not interchangeable and that the mechanism selection is an essential element of RSM's high performance.



\subsection{Mechanisms specialize in modeling different transitions} \label{se:independent_mech}
\input{figures/full_step_main_2.tex}

\input{figures/full_step_main_3.tex}

To continue clarifying hypothesis 1 and start analyzing hypothesis 2, in Figure \ref{fig:fullsteps_main}, we study the role of each mechanism in RSM.
The RSM reconstruction results are presented in the second row, whereas, in the last five rows, a single mechanism is assigned to all slots for all of the 10 roll-out prediction steps.
The analysis shows that RSM not only produces a reasonable reconstruction compared to the ground-truth frame but also encourages the mechanisms to distinguish themselves in the roles they take. 
In this sample, we have the 5 slots corresponding to:
1: red round,
2: blue triangle,
3: green square,
4: purple round,
and 5: yellow triangle.

Looking deeper into the reconstruction result, RSM takes advantage of the CCI to assign a suitable mechanism for each slot in all scenarios.
More specifically, there are three scenarios of objects in 2D Shapes: 
(1) \textbf{\textit{Allowed to move}} as in steps $0 \rightarrow 1$ and $1 \rightarrow 2$;
(2) \textbf{\textit{Blocked by the wall}} as in steps $2 \rightarrow 3$, $3\rightarrow 4$; 
and (3) \textit{\textbf{Blocked by an object}} that occupies the desired destination as in step $4\rightarrow 5$.
RSM predicts the movement (to the right) of the yellow triangle accurately in the first case and predicts the \textit{zero} changes of slots and preserves the system status due to no movement happening in cases 2 and 3.

From the visualization, we find that the mechanisms specialize with respect to the action: Mechanism 1: $\mathsf{RIGHT}$, Mechanism 2: $\mathsf{UP}$, Mechanism 3: $\mathsf{LEFT}$, Mechanism 4: \textit{DO NOT MOVE}, and Mechanism 5: $\mathsf{DOWN}$.
However, for the same action, RSM considers the particular situation and reacts differently.
For instance, with the same action $\mathsf{UP}$ given in step 1 (green bounding box) on the green rectangle and step 3 (red bounding box) on the red round, RSM recognizes the situations that the object is allowed to move and blocked by the upper wall, respectively, then applies the movement at step 1 while not modifying objects at step 3 and generating the correct reconstruction in both cases.
We can see a similar example in the row of mechanism 2 at step 3 $\rightarrow$ 4 (cyan bounding box) when the green object does not move $\mathsf{UP}$ but remains at the same position since it is blocked by the red object.

NPS enables a $\mathsf{null}$ rule to produce \textit{zero} change of the primary slot.
RSM achieves the same without any artificially defined procedure: it implicitly recognizes the possibility of \textit{zero} modification of a slot, then assigns the procedure of \textit{DO NOT MOVE} to a particular mechanism, as demonstrated by mechanism 4 in Figure \ref{fig:fullsteps_main}.

Appendix \ref{ap:mech_fulls} provides the visualization of the entire 10 roll-out steps of the 2D Shapes and Balls environments.


\input{figures/ablation_main.tex}

\subsubsection{The ability to decompose the visual frame into slots}

\input{figures/disentanglement_ability_extraction.tex}
\input{figures/disentanglement_ability_reconstruction.tex}


We conduct a qualitative comparison to clarify hypothesis 3 about the effectiveness of RSM in the slot-centric representation learning task.
In Figure \ref{fig:feature_maps}, we illustrate a comparison of the extracted feature maps with a size of $\mathsf{10 \times 10}$, which are constructed by the $\mathsf{Encoder}$ model.
Afterward, in Figure \ref{fig:reconstruct_slots}, we illustrate the reconstructed slots and frame with a size of $\mathsf{3} \times \mathsf{50} \times \mathsf{50}$, which are acquired by the $\mathsf{Decoder}$ model that receives the input as the predicted next state.
We find that RSM decomposes objects in the input frame into separated slots and keeps each object in the same slot until they are decoded.
In contrast, the baselines do not capture all objects,  they produce noised feature maps (MBRL), or put the same object in two slots and identify two objects in another slot (NPS).

We observe that the combination of the CCI with the sequential updates that encourage slots to observe the modification of each other benefits from recognizing the overlap of objects.
More specifically, RSM only generates a part of the object in case that object is covered by another one (\eg the green and blue cubes in slot 2 and slot 4 are partially covered by the yellow cube).
On the other hand, the reconstructed frames by the baselines overlook the information of the objects' visible order, generating overlapped objects in some cases (\eg the green, blue, and yellow cubes in MBRL overlapped to each other).
We further discuss this conclusion in Appendix \ref{ap:reconstructions} and \ref{ap:ab}.


\section{Experiment Details}

% \input{figures/decompose_slots/Pong.tex}

\subsection{Environment details} \label{ap:envs}
\subsubsection{Predict the next steps in Atari games}
We explore the Atari 2600 environments, which are commonly used in \cite{Kipf2020Contrastive, goyal2021recurrent, NEURIPS2021_10907813}.
The challenge of this kind of environment is that multiple factors cause the movements in two consecutive time steps; however, the given action has only affected the movement of a single object.
For instance, there are 3 factors in Pong, which are (1) the ball follows physics rules to keep moving towards or collide with the walls or the two paddles, (2) the green paddle is controlled by the given action, (3) the white paddle that follows the movement of the ball.

Following \cite{Kipf2020Contrastive, NEURIPS2021_10907813} in the OOD test set generation, we set up the variable $\mathsf{warmstart}$ that designates the number of frames to be discarded from the beginning before recording the game.
Afterward, we use the same $\mathsf{warmstart}$ to produce the train, evaluation, and the iid test set while using another value of $\mathsf{warmstart}$ to generate the OOD test set.

\subsubsection{Manipulations in grid world}
This dataset contains a number of objects placed in a $\mathsf{5 \times 5}$ grid.
At each time step, given a single frame and an action that specifies one object and one manipulation from $\mathsf{UP}$, $\mathsf{RIGHT}$, $\mathsf{DOWN}$, and $\mathsf{LEFT}$.
The challenge of this task is to consider the feasibility of the given action and predict the next frame.
For instance, moving an object to $\mathsf{LEFT}$ is executable if there is no object occupied on the left of that object; otherwise, the frame is not changed.

For both 2D Shapes and 3D Cubes, we generate 5 objects for iid sets and 3 objects for the OOD test set.

\subsubsection{Movements in physics simulation}
We investigate the physic simulation environment introduced by \cite{Kipf2020Contrastive}, containing three balls moving by the same and unchanged velocities in a 2D plane.
Different from the rest of the environments in this study, the environment Balls is not governed by any given action. 
The challenge of this task is to recognize the latent velocities at the beginning time and generate the next step with the constant movement of objects.

The ball radius equals $\mathsf{4}$ in the training set and iid test set, while the ball radius is set to $\mathsf{5}$ in the evaluation set and $\mathsf{3}$ for the OOD test set.

% \subsubsection{Evaluation Metrics}

% We report the mean and standard error over 30 runs at 1, 5, and 10 prediction steps into the future.

\subsection{Encoder and Decoder architecture}

\subsubsection{Encoder Architecture}
In this work, we follow the encoder architecture from baselines \cite{Kipf2020Contrastive, BENCHMARKS2021_8f121ce0, NEURIPS2021_10907813} that contains 2 components:
\begin{itemize}
    \item Object Extractor: CNN layers that extract the visual input to $N$ feature maps.
    \item Object Encoder: MLP layers to encoding feature maps to vector space, \textit{i.e.} the object slots.
\end{itemize}

Afterward, an $\mathsf{Encoder}$ model consists of a single Object Extractor and a single Object Encoder.


\subsubsection{Decoder Architecture}
\begin{figure*}[t]%
\centering
\includegraphics[width=0.6\linewidth]{figures/method/decoder.pdf}
\caption{\textbf{Decoder architecture} contains a list of $N$ CNN-based decoders corresponding to $N$ slots that share the same structure. The frame reconstruction is obtained by the sum of $N$ slot reconstructions.}%
\label{fig:decoder}%
\end{figure*}

We construct a new architecture for the Decoder working on slot-based visual prediction tasks.
We propose the Slot Decoder that decodes a single slot to frame.
$$s'_n^{t+1} \in \mathbb{R}^{d_s} \rightarrow \text{Slot Decoder} \rightarrow \text{slot reconstruction} \in \mathbb{R}^{\mathsf{3 \times 50 \times 50}}$$
Then, a $\mathsf{Decoder}$ model consists of $N$ Slot Decoders that share the same architecture but different weights.

Figure \ref{fig:decoder} provides the overview of the proposed decoder architecture.
Specifically, each slot in the latent space is passed through a corresponding Slot Decoder model to produce an RGB slot reconstruction.
Finally, the frame reconstruction is obtained by the sum of $N$ slots reconstruction with a size of $\mathsf{3 \times 50 \times 50}$.

In this study, we use the described architecture for the proposed method and baselines.


\subsection{Loss Functions}

\subsubsection{Contrastive Loss During Training the encoder and transition model}

In this study, we follow the same Contrastive loss setup as \cite{Kipf2020Contrastive}, which is also used in all of the baselines. In this setup, we use the prediction result of the model to form the positive hypothesis, whereas, we sample random input states in the same batch to form the negative hypothesis.

Mathematically, the Contrastive loss function can be described as follow:
\begin{equation} \label{loss_function}
\begin{aligned} 
H &= \mathsf{MSE}(\boldsymbol{s}^{'}_{t+1}, \boldsymbol{s}_{t+1}) \\ 
\tilde{H} &= \mathsf{MSE}(\tilde{\boldsymbol{s}}_{t+1}, \boldsymbol{s}_{t+1})  \\
Contrastive\ Loss: \mathcal{L} &= H + \mathsf{max}(0, \gamma - \tilde{H}) \\
\end{aligned}
\end{equation}
where $\boldsymbol{s}_{t+1}$ denotes the abstract target state obtained by passing the target observation ($x_{t+1}$) through $encoder$, $\boldsymbol{s}^{'}_{t+1}$ represent the abstract next state output by the transition model, and $\tilde{\boldsymbol{s}}_{t+1}$ indicates the random abstract state in the training batch of data.
$\gamma$ is a hyper-parameter which is set to $1$ by following \cite{Kipf2020Contrastive}.

\subsubsection{Binary Cross Entropy in Training the Decoder}

We consider two $\mathsf{BCE}$ loss terms in training $\mathsf{Decoder}$, $\mathcal{L}_1$ and $\mathcal{L}_2$, as mathematically described in \cref{loss_dec_function}.
More specifically, $\mathcal{L}_1$ is computed by passing $s_t$ through $\mathsf{Decoder}$ to achieve $x^{'}_t$ which is expected to close to $x_t$.
$\mathcal{L}_1$ follow the same procedure that is passing the output of the transition model, the abstract states $s^{1}_{t+1}$, to achieve the prediction of next frames, $x^{'}_{t+1}$, that is desired to close to the observation at time $t+1$, denoted as $x_{t+1}$. 
Then, the final $\mathsf{BCE}$ loss for the $\mathsf{Decoder}$ training is formularized as in \cref{loss_dec_function}.

\begin{equation} \label{loss_dec_mat}
\begin{aligned} 
\boldsymbol{x}^{'}_{t} &= \mathsf{Decoder}(\boldsymbol{s}_{t}) \\ 
\boldsymbol{x}^{'}_{t+1} &= \mathsf{Decoder}(\boldsymbol{s}^{'}_{t+1}) \\ 
\end{aligned}
\end{equation}

\begin{equation} \label{loss_dec_function}
\begin{aligned} 
\mathcal{L}_1 &= \mathsf{BCE}(\boldsymbol{x}^{'}_{t}, \boldsymbol{x}_{t}) \\ 
\mathcal{L}_2 &= \mathsf{BCE}(\boldsymbol{x}^{'}_{t+1}, \boldsymbol{x}_{t+1})  \\
BCE\ Loss: \mathcal{L}_{Decoder} &= \mathcal{L}_1 + \mathcal{L}_2 \\
\end{aligned}
\end{equation}

\subsection{Ranking based Evaluation Metrics - Hits at Rank 1 (H@1)} \label{ap:metrics}
% \subsubsection{}
We follow the ranking-based metrics in latent spaces used in \cite{Kipf2020Contrastive, goyal2020object, goyal2021recurrent, BENCHMARKS2021_8f121ce0}, which is the Hit at rank 1 (H@1).
This metric is introduced by \cite{Kipf2020Contrastive} with the definition of one hit when the predicted state representation is nearest to the encoded observation.
We report the average number of hits over the test set.
The higher H@1 score indicates a better model prediction.

% \subsubsection{Mean Reciprocal Rank (MRR)}
% MRR is computed as: 
% $$MRR = \frac{1}{N} \sum^N_{n=1} \frac{1}{rank_n}$$
% which is defined as an average inverse rank, where $rank_n$ is the rank of $n^{th}$ sample when ranking is done over all reference state representations.
% The higher value of MRR demonstrates better performance.

\section{Reproducibility}

\begin{table}[!h]
\begin{center}
\small
\begin{tabular}{ |c|c|c|c|c|c|c|c| } 
 \hline
 Environment & Data points & Input frames & \#Slots & Action Space & Epochs & \#Mechanisms  \\ \hline
 2D Shapes & 1k/10k/10k & 1 & 5 & 4 & 100 & 5 \\ 
 3D Cubes & 1k/10k/10k & 1 & 5 & 4 & 100 & 5\\
 Breakout & 1k/100/100 & 2 & 3 & 4 & 200 & 5 \\
 Pong & 1k/100/100 & 2 & 3 & 6 & 200 & 3 \\ 
 Balls & 5k/1k/1k & 2 & 3 & 0 & 100 & 7\\\hline
 PHYRE & 5k/1k/1k & 2 & 3 & 0 & 100 & 7\\
 Physion & 5k/1k/1k & 2 & 3 & 0 & 100 & 7\\\hline
\end{tabular}
\caption{\label{tab:hyper} \textbf{Hyperparameters indication}. The number of Data points represents the size of the Train/Validation/Test sets, \textit{k} abbreviated for 1000. The number of Mechanisms represents the chosen amount after validating.}
\end{center}
\end{table}

\subsection{Datasets Generation} \label{ap:reproduce_data}

Follow \cite{Kipf2020Contrastive} a random policy is applied during generating datasets.
The size of the training, validating, and test sets (the same for the iid and OOD test sets) are indicated in the second columns of Table \ref{tab:hyper}.

As mentioned in Appendix \ref{ap:envs}, we adjust the $\mathsf{warmstart}$ to generate the iid and OOD data sets for Atari games.
For Pong, the $\mathsf{warmstart}$ is set to 58 and 100 for the iid and OOD data sets, respectively.
The $\mathsf{warmstart}$ pair for Breakout is 50 and 100.
% For 2D Shapes and 3D Cubes, we simply adjust the configuration of the number of objects, which are 3 objects for the OOD test sets and 5 for the rest of the data sets.
% For Balls, we set the 


\subsection{Hyper-parameters}
Most of the hyper-parameters used in this work are followed by C-SWM \cite{Kipf2020Contrastive}.
The rest of Table \ref{tab:hyper} summarizes the hyper-parameters for training and environment configurations.
In addition, for all environments and methods, using the Adam optimizer \cite{DBLP:journals/corr/KingmaB14}, a learning rate of $\mathsf{5e-4}$, batch size 1024, and hidden size 512.
Follows \cite{Kipf2020Contrastive}, each slot is encoded into a $4-dimension$ vector. 
After training the $\mathsf{Encoder}$ and the transition model, we train the $\mathsf{Decoder}$ for 100 epochs.

For the number of mechanisms in RSM, we trained models with 3, 5, and 7 mechanisms. Then, the chosen number is decided based on the result of the validation set over 30 random seeds.
This number is the same for the reported iid and OOD results and could differ among environments.
In addition, in Appendix \ref{ap:num_mech}, we further analyze the model performance in different numbers of mechanisms.


\section{Further discussion on the performance of each mechanism} \label{ap:mech_fulls}

% \subsubsection{Difference among mechanisms and the importance of mechanisms selection}

% \input{figures/random_mechanisms.tex}
% To clarify the first hypothesis about the specialized knowledge in each mechanism, in Figure \ref{fig:random_mechanisms}, we provide the H@1  performance comparison in two cases: the mechanism assignment produced by RSM (at Step 2) and from a random selection, which yields very poor results, especially for a larger number of steps.

% The analysis demonstrates that (1) mechanisms learned distinct and significantly differentiated knowledge and (2) assigning proper mechanisms to slots is essential to gain a high ranking score, which supports our hypothesis 1.

\subsection{Observation on 2D Shapes}

% \input{figures/full_steps.tex}
\input{figures/full_steps_2.tex}
In Figure \ref{fig:fullsteps}, we provide 10 steps which is the extended version of the analysis in Section \ref{se:independent_mech}.
The analysis demonstrates the ability of RSM to generate correct reconstruction frames over 10 rolling-out prediction steps.
The figure also exposure the stability of RSM in handling the required action in all cases of objects being allowed to move or being blocked by another object or one of the 4 walls.

Moreover, the analysis witnesses the strong points of mechanisms to learn distinct knowledge and consider well the particular situation to produce a proper actual response.
For instance, the action moving to the $\mathsf{LEFT}$ is provided in steps 2 and 7 in cases where the purple round object is free to move at step 7 while the blue rectangle is blocked by the wall at step 2 and is not allowed to move.
As we can see from the figure, mechanism 3 takes the manipulation $\mathsf{LEFT}$ but generates different actual movements on these 2 steps.
In particular, mechanism 3 creates a \textit{zero} modification to step 2 and moves the purple object to the left accurately.

However, it seems to be sensitive in cases of objects being blocked by another object in the last 5 rows when a single mechanism is applied to all slots at each prediction step.
One reason comes from the difference in evaluation settings, there is only at most 1 slot is moved in the conventional flow during training and testing, while in this analysis, all slots are moved after each prediction step.

\subsection{Observation on Balls}

In Figure \ref{fig:fullsteps_balls}, we illustrate the transformation of slots that are not governed by any action in Balls.
First of all, RSM generates reasonable reconstructions over 10 steps prediction into the future, which are illustrated in row 3$^{th}$.
We observe that in different seeds and methods, slots in Balls capture the 3 balls and a circular trajectory.
Next, looking at frame reconstructions with a single mechanism applied to all slots, we can see that all reconstructed frames are not suitable due to the missing objects or not correcting the object's position compared to the ground-truth frame.
Lastly, the following points describe some observations on the actual transformation produced by mechanisms from the reconstruction generated by a single mechanism:

\input{figures/full_steps_balls.tex}
\textbf{Observation 1}: mechanism performs a constant movement of slot-entity. 
Clearly illustrated in the figure, during 10 steps, slots do not change direction and seem to preserve the same velocities.
However, directions and velocities are different among slots and mechanisms.
Specifically, the circular trajectories move up or to some frame's corner (upper); the groups of colored entities keep rotating by a pair of velocities in the 2D plane.

\textbf{Observation 2}: mechanism's performance is different when applied to different slots.
As we can see from the transformation of slots when mechanism 1 is applied, the circular trajectory in slot 1 keeps moving to the upper-right corner, whereas, slot 2 rotates counterclockwise and slot 3 slightly rotates or even does not move.

% \textbf{Observation 3}: in different data points, the entities balls are actively governed by different mechanisms.
% In this example, slots 2 and 3, which contain

These observations not only encourage our hypothesis 2 that mechanisms learn different and meaningful knowledge but also demonstrate the reusability of mechanisms in RSM.

\input{figures/mechs.tex}

\section{Reconstruction Results} \label{ap:reconstructions}

% \subsection{Reconstruction in 2D Shapes environment}
\input{figures/reconstruct_Shapes_appendix.tex}

% In Figures \ref{fig:feature_maps_2d}, we illustrate the comparison of object extraction in the 2D Shapes environment among slot-based methods.
% Besides, in Figure \ref{fig:reconstruct_shapes}, we compare the reconstructed frames of all methods.



\subsection{Reconstruction in 3D Cubes environment}
\input{figures/reconstruct_Cubes_appendix}

One of the challenges to generating reconstructions in 3D Cubes environment is to recognize the visibility order of objects.
As visualized in Figure \ref{fig:reconstruct_cubes}, RSM exposures the strength in communication among slots to obtain the order information, as well as generate the proper movement of slots and achieve an accurate reconstruction compared to the ground-truth.
In contrast, MBRL misses that kind of information from the beginning steps and renders the blue, green, and yellow objects inside each other, then, witnesses a huge gap from the following steps to step 10.
Besides, other methods lose the information of some objects and produce a not completed reconstruction at the end.

% \subsection{Reconstruction in Breakout environment}

\input{figures/reconstruct_Pong_appendix}
% Figure \ref{fig:reconstruct_breakout} compare the reconstruction result in a 

% We find that method that only makes the changes in one slot as NPS makes it difficult to control the environments, such as Breakout, that require the adaptability to the modification of other slots.

\subsection{Reconstruction in Pong environment}
\input{figures/reconstruct_Breakout_appendix}
\input{figures/reconstruct_Balls_appendix}

Figure \ref{fig:reconstruct_pong} provides a problematic test case that contains a collision between the ball and the green paddle from step 1 to step 3, and the ball changes the movement direction in step 2.
As illustrated in the figure, RSM produces the best reconstruction for the whole of 10 steps, which proves the benefit of information integration among slots in complex cases.
More specifically, RSM recognizes and manages the collision well, and then, maintains the uniform motion of the ball after collision till the last step while handling the actions applied on the green paddle.
MBRL also renders the three objects in Pong at the first 2 steps; however, it generates a ball that is blurred from step 3 and becomes hard to see at step 10.
Other methods do not recognize the ball from the first step and show the loss of either the white or green paddle from step 7.

% \subsection{Reconstruction in Balls environment}

\input{figures/slots_cube_ap.tex}


\section{Ablation Studies} \label{ap:ab}


We conduct ablation studies to emphasize the benefit of the communication flow proposed in RSM.
As described in Section \ref{se:ab_main}, the ablation studies in this work are listed as follows:
\begin{itemize}
    \item RSM $\mathsf{ab\ 01}$: the CCI is not used at step 2 but is used at step 3.
    \item RSM $\mathsf{ab\ 10}$: the CCI is used at step 2 but is not used at step 3.
    \item RSM $\mathsf{ab\ 00}$: the CCI is used at neither step 2 nor step 3.
    \item RSM $\mathsf{ab\ par}$: the CCI is used at both step 2 and step 3, but wrapped in parallel updates instead of sequential order.
    \item MLP-CCI: the CCI is computed by an MLP instead of $\mathsf{MultiheadAttention}$, then is used at both step 2 and step 3 in a sequential manner.
\end{itemize}

Table \ref{ta:ab_full} represents the full comparison of the original design of RSM and the ablations.
Overall, the results show that RSM exposure has the strongest result in both iid and OOD.

In addition, Figure \ref{fig:reconstruct_slots_par} provides the comparison of RSM and the absence of sequential information integration.

\input{tables/usage_ctx.tex}



==> sections/result_main.tex <==



==> tables/ab_attn_weight.tex <==
\begin{figure}[h]
\centering
\small
\begin{Overpic}[abs,unit=1mm,grid=false,tics=3]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}}
      Rollout & Gold & Pred & Slot 1 & Slot 2 & Slot 3 & Slot 4 & Slot 5 & Slot 6 & Slot 7 & Slot 8 \\
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step06.pdf}}
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step06.pdf}} 
     \\ 
    $t = 0$ & \\
     $\dots$ & \\ \\[-4.9pt]
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step06.pdf}}
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step06.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step06.pdf}} 
     \\ 
    $t = 6$ & \\
     & \\ \\[-4.9pt]
     Mechanism & &
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot1.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot2.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot3.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot4.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot5.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot6.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot7.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step6_slot8.pdf}} 
     \\ \\[-9.9pt]
    & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step07.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step07.pdf}} 
     & \\ 
    $t=7$ & & & & & & & \\
    & \\ \\[-4.9pt]
    Mechanism & & 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot1.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot2}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot3.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot4.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot5.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot6.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot7.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step7_slot8.pdf}} 
     & \\ \\[-9.9pt]
    & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step08.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step08.pdf}} 
     & \\
     $t=8$ & \\ 
     & \\ \\[-4.9pt]
     Mechanism & & 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot1.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot2.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot3.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot4.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot5.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot6.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot7.pdf}} 
     & \multirow{1}{0.05\textheight}{\includegraphics[width=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/mechs/PHYRE_dp22_step8_slot8.pdf}} 
      & \\ \\[-9.9pt]
    & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step09.pdf}} 
     & \\
     $t=9$ & \\
     $\dots$ \\ \\[-4.9pt]
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/GT/PHYRE_slotformer_dp22_gt_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_pred_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0001_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0002_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0003_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0004_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0005_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0006_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0007_step09.pdf}} 
     & \multirow{3}{0.05\textheight}{\includegraphics[height=0.05\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp22_slot0008_step09.pdf}} 
     & \\
     $t=14$ & \\
     & \\
  \end{tabular}}%

% \put(0,0){\color{red}\linethickness{1pt} \polygon(83, 21.75)(83, 19)(88.5,19)(88.5,21.75)}  %step 0->1
% \put(0,0){\color{yellow}\linethickness{1pt} \polygon(35.4, 21)(35.4, 16.7)(42, 16.7)(42, 21)}  %step 0->1

\end{Overpic}
\caption{\textbf{Action planning task and the undergoing decision-making on mechanisms assignment in PHYRE}. RSM disentangles objects' dynamics into reusable mechanisms, which can be expressed as (1) Overall observing, (2) Colliding, (3) Moving left or right, (4) Idle, and (5) Falling down.}
\label{fig:fullsteps_main_attn}
\end{figure}




==> tables/ap_physion.tex <==
\begin{figure}[t]
\centering
\begin{Overpic}[abs,unit=1mm,grid=yes,tics=3]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}cc}
    Rollout step= & 0 & 10 & \textbf{20} & \textbf{30} & \textbf{40} & 49 & Remarks\\
     & 
     \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step00.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step10.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step20.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step30.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step40.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step49.pdf}} 
     \\ 
    Gold & \\
    & \\ \\[-4pt]
    & 
     \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/gt/Physion_slotformer_dp12_gt_step00.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/rsm/Physion_rsm_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/rsm/Physion_rsm_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/rsm/Physion_rsm_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/rsm/Physion_rsm_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/rsm/Physion_rsm_dp12_pred_step49.pdf}} 
     & Accurate dynamics \\ 
    \textbf{RSM (Ours)} & & & & & & & Sharpness preserved\\
    & \\ \\[-4pt]
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step00.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/nps/Physion_NPS_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/nps/Physion_NPS_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/nps/Physion_NPS_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/nps/Physion_NPS_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/nps/Physion_NPS_dp12_pred_step49.pdf}} 
     & Incorrect dynamics \\ 
     NPS & & &  & & & & Changed shapes\\ 
     & \\ \\[-4pt]
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step00.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step49.pdf}} 
     & Incorrect dynamics \\ 
    SlotFormer & &  & & & & & Lost sharpness\\
    & \\ \\[-4pt]
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/slotforme/Physion_slotformer_dp12_pred_step00.pdf}} 
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/switch/PHYRE_slotformer_dp12_switch_step10.pdf}} 
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/switch/PHYRE_slotformer_dp12_switch_step20.pdf}} 
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/switch/PHYRE_slotformer_dp12_switch_step30.pdf}} 
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/switch/PHYRE_slotformer_dp12_switch_step40.pdf}} 
    & \multirow{3}{0.06\textheight}{\includegraphics[height=0.06\textheight]{rsm2/rollout_vis/obj3d/switch/PHYRE_slotformer_dp12_switch_step49.pdf}} 
     &  Incorrect dynamics \\ 
    SwitchFormer & \\
    & \\ \\[-4pt]
  \end{tabular}}%

% slotformer
% \put(0,0){\color{red}\linethickness{1pt} \polygon(70.3, 17.6)(70.3, 14.5)(76,14.5)(76, 17.6)}  %step 0->1
% % \put(0,0){\color{red}\linethickness{0.1pt} \polygon(60, 22)(60, 18)(64,18)(64, 22)}  %step 0->1
% \put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(41, 16.75)(41, 13.5)(48,13.5)(48,16.75)}  %step 0->1

% % % switch
% \put(0,0){\color{red}\linethickness{0.1pt} \polygon(51.6, 8)(51.6, 2)(54.9, 2)(54.9, 8)}  %step 0->1
% % \put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(35.4, 9)(35.4, 5)(42, 5)(42, 9)}  %step 0->1

% % % nps
% \put(0,0){\color{red}\linethickness{1pt} \polygon(51, 27.0)(51, 23.5)(57.0,23.5)(57,27.0)}  %step 0->1
% \put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(68.6, 27.1)(68.6, 24.7)(71, 24.7)(71, 27.1)}

% \put(0,0){\color{blue}\linethickness{0.1pt} \polygon(39.6, 48.2)(39.6, 0.0)(68.1, 0.0)(68.1, 48.2)}  %step 0->1

\end{Overpic}
\caption{\textbf{Comparison of rollout frames in Physion}. RSM generates frames with precise dynamics and maintains visual quality, even during complex actions in steps 20 to 40. In contrast, the baselines produce ones with artifacts (yellow boxes) and inaccurate dynamics (red boxes).}
\label{fig:fullsteps_main}
% \vspace{-5mm}
\end{figure}




==> tables/iid_main.tex <==
\begin{table*}[t]
\caption{Comparison between the proposed RSM and the baselines in IID setting. Number denotes ranking scores in percentage (\%) for multi-step prediction into the future in latent space. The reported scores are mean and Standard Error over 30 runs. The higher results indicate the better in prediction. The best scores are \textbf{bolded}. }
\label{table:iid_result}
\begin{center}
\begin{tabular}{llcccccc}
\hline & \\[-10pt]
& & \multicolumn{2}{c}{\textit{1 step}} & \multicolumn{2}{c}{\textit{5 steps}} & \multicolumn{2}{c}{\textit{10 steps}} \\ \hline & \\[-1.0em]
& \textit{\textbf{}} & \textbf{H@1} & \textbf{MRR} & \textbf{H@1} & \textbf{MRR} & \textbf{H@1} & \textbf{MRR} \\
\hline & \\[-10pt] 
\multirow{4}{9pt}{\rotatebox{90}{\textbf{Shapes}}} 
& C-SWM & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0}\\
& MBRL & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.8\textcolor{lightgray}{±0.0} & 99.9\textcolor{lightgray}{±0.0} & 98.0\textcolor{lightgray}{±0.1} & 98.8\textcolor{lightgray}{±0.1}\\
& NPS & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.7\textcolor{lightgray}{±0.1} & 99.8\textcolor{lightgray}{±0.1} & 97.0\textcolor{lightgray}{±0.3} & 98.1\textcolor{lightgray}{±0.2}\\
& RSM (Ours) & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.9\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & 97.9\textcolor{lightgray}{±0.1} & 98.7\textcolor{lightgray}{±0.1}\\
\hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Cubes}}} 
& C-SWM & \textbf{100.0}\textcolor{lightgray}{±0.2} & \textbf{100.0}\textcolor{lightgray}{±0.1} & \textbf{99.6}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{98.2}\textcolor{lightgray}{±0.5} & \textbf{99.8}\textcolor{lightgray}{±0.6}\\
& MBRL & 99.8\textcolor{lightgray}{±0.1} & 99.9\textcolor{lightgray}{±0.0} & 99.1\textcolor{lightgray}{±0.2} & 99.5\textcolor{lightgray}{±0.1} & 96.5\textcolor{lightgray}{±0.4} & 97.8\textcolor{lightgray}{±0.3}\\
& NPS & 99.8\textcolor{lightgray}{±0.2} & 99.9\textcolor{lightgray}{±0.1} & 99.1\textcolor{lightgray}{±0.6} & 99.5\textcolor{lightgray}{±0.3} & 96.6\textcolor{lightgray}{±1.6} & 97.9\textcolor{lightgray}{±1.0}\\
& RSM (Ours) & 99.8\textcolor{lightgray}{±0.0} & 99.9\textcolor{lightgray}{±0.0} & 99.2\textcolor{lightgray}{±0.6} & 99.6\textcolor{lightgray}{±0.4} & 93.9\textcolor{lightgray}{±1.5} & 98.8\textcolor{lightgray}{±1.1}\\\hline 
& \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Breakout}}} 
& C-SWM & 65.6\textcolor{lightgray}{±4.1} & 76.9\textcolor{lightgray}{±2.9} & 36.7\textcolor{lightgray}{±3.7} & 50.7\textcolor{lightgray}{±3.3} & 21.8\textcolor{lightgray}{±2.2} & 34.0\textcolor{lightgray}{±2.4}\\
& MBRL & 64.7\textcolor{lightgray}{±1.2} & 73.2\textcolor{lightgray}{±0.7} & 37.4\textcolor{lightgray}{±1.8} & 49.8\textcolor{lightgray}{±1.7} & 14.9\textcolor{lightgray}{±2.1} & 27.1\textcolor{lightgray}{±2.6}\\
& NPS & 68.0\textcolor{lightgray}{±0.3} & 79.4\textcolor{lightgray}{±1.2} & 44.5\textcolor{lightgray}{±1.1} & 58.6\textcolor{lightgray}{±1.2} & \textbf{27.2}\textcolor{lightgray}{±1.5} & 39.3\textcolor{lightgray}{±2.5}\\
& RSM (Ours) & \textbf{73.3}\textcolor{lightgray}{±1.0} & \textbf{82.7}\textcolor{lightgray}{±0.6} & \textbf{46.6}\textcolor{lightgray}{±1.7} & \textbf{59.9}\textcolor{lightgray}{±1.4} & \textbf{27.2}\textcolor{lightgray}{±2.0} & \textbf{40.0}\textcolor{lightgray}{±1.9}\\
\hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Pong}}} 
& C-SWM & 44.2\textcolor{lightgray}{±4.9} & 61.7\textcolor{lightgray}{±4.0} & 21.4\textcolor{lightgray}{±1.9} & 38.4\textcolor{lightgray}{±2.5} & 15.2\textcolor{lightgray}{±1.7} & 30.3\textcolor{lightgray}{±2.5}\\
& MBRL & 50.3\textcolor{lightgray}{±2.0} & 63.8\textcolor{lightgray}{±1.5} & 23.9\textcolor{lightgray}{±1.5} & 40.2\textcolor{lightgray}{±1.5} & 16.8\textcolor{lightgray}{±2.1} & 31.0\textcolor{lightgray}{±2.3}\\
& NPS & 52.0\textcolor{lightgray}{±5.0} & 67.9\textcolor{lightgray}{±3.5} & 24.2\textcolor{lightgray}{±1.6} & 41.4\textcolor{lightgray}{±1.9} & 15.4\textcolor{lightgray}{±2.2} & 32.2\textcolor{lightgray}{±2.4}\\
& RSM (Ours) & \textbf{53.9}\textcolor{lightgray}{±1.5} & \textbf{69.6}\textcolor{lightgray}{±1.0} & \textbf{30.6}\textcolor{lightgray}{±1.0} & \textbf{48.1}\textcolor{lightgray}{±0.8} & \textbf{23.5}\textcolor{lightgray}{±0.7} & \textbf{40.6}\textcolor{lightgray}{±0.7}\\
\hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Balls}}} 
& C-SWM & 99.7\textcolor{lightgray}{±0.1} & \textbf{99.9}\textcolor{lightgray}{±0.1} & 86.6\textcolor{lightgray}{±4.9} & 91.8\textcolor{lightgray}{±3.1} & 64.9\textcolor{lightgray}{±8.8} & 74.8\textcolor{lightgray}{±7.1}\\
& MBRL & 99.8\textcolor{lightgray}{±0.1} & \textbf{99.9}\textcolor{lightgray}{±0.1} & 89.7\textcolor{lightgray}{±4.5} & 93.7\textcolor{lightgray}{±3.1} & 68.1\textcolor{lightgray}{±6.0} & 78.6\textcolor{lightgray}{±5.1}\\
& NPS & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{99.9}\textcolor{lightgray}{±0.0} & 89.5\textcolor{lightgray}{±1.9} & 94.2\textcolor{lightgray}{±1.6} & \textbf{73.2}\textcolor{lightgray}{±3.3} & \textbf{84.0}\textcolor{lightgray}{±1.1}\\
& RSM (Ours) & 99.8\textcolor{lightgray}{±0.0} & \textbf{99.9}\textcolor{lightgray}{±0.0} & \textbf{92.9}\textcolor{lightgray}{±1.8} & \textbf{96.1}\textcolor{lightgray}{±1.1} & 72.6\textcolor{lightgray}{±4.5} & 82.2\textcolor{lightgray}{±3.3}\\
\hline \\
\end{tabular}
\end{center}
\end{table*}


==> tables/obj3d_new.tex <==
\begin{figure}[t]
\centering
\begin{Overpic}[abs,unit=1mm,grid=yes,tics=3]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}cc}
    Rollout step= & 0 & 10 & \textbf{20} & \textbf{30} & \textbf{40} & 49 & Remarks\\
     & 
     \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_SwitchFormer_dp12_gt_step00.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_SwitchFormer_dp12_gt_step10.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_slotformer_dp12_gt_step20.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_slotformer_dp12_gt_step30.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_slotformer_dp12_gt_step40.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_slotformer_dp12_gt_step49.pdf}} 
     \\ 
    Gold & \\
    & \\ \\[-16pt]
    & 
     \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/gt/OBJ3D_new_slotformer_dp12_gt_step00.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/rsm/OBJ3D_new_rsm_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/rsm/OBJ3D_new_rsm_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/rsm/OBJ3D_new_rsm_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/rsm/OBJ3D_new_rsm_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/rsm/OBJ3D_new_rsm_dp12_pred_step49.pdf}} 
     & Accurate dynamics \\ 
    \textbf{RSM (Ours)} & & & & & & & Sharpness preserved\\
    & \\ \\[-16pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step00.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/nps/OBJ3D_new_NPS_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/nps/OBJ3D_new_NPS_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/nps/OBJ3D_new_NPS_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/nps/OBJ3D_new_NPS_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/nps/OBJ3D_new_NPS_dp12_pred_step49.pdf}} 
     & Incorrect dynamics \\ 
     NPS & & &  & & & & Changed shapes\\ 
     & \\ \\[-16pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step00.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step10.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step20.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step30.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step40.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/slotforme/OBJ3D_new_slotformer_dp12_pred_step49.pdf}} 
     & Incorrect dynamics \\ 
    SlotFormer & &  & & & & & Lost sharpness\\
    & \\ \\[-16pt]
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step00.pdf}} 
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step10.pdf}} 
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step20.pdf}} 
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step30.pdf}} 
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step40.pdf}} 
    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/obj3d/switch/OBJ3D_new_SwitchFormer_dp12_pred_step49.pdf}} 
     &  Incorrect dynamics \\ 
    SwitchFormer & \\
    & \\ \\[-16pt]
  \end{tabular}}%

% slotformer
\put(0,0){\color{red}\linethickness{1pt} \polygon(70.3, 17.6)(70.3, 14.5)(76,14.5)(76, 17.6)}  %step 0->1
% \put(0,0){\color{red}\linethickness{0.1pt} \polygon(60, 22)(60, 18)(64,18)(64, 22)}  %step 0->1
\put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(41, 16.75)(41, 13.5)(48,13.5)(48,16.75)}  %step 0->1

% % switch
\put(0,0){\color{red}\linethickness{0.1pt} \polygon(51.6, 8)(51.6, 2)(54.9, 2)(54.9, 8)}  %step 0->1
% \put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(35.4, 9)(35.4, 5)(42, 5)(42, 9)}  %step 0->1

% % nps
\put(0,0){\color{red}\linethickness{1pt} \polygon(51, 27.0)(51, 23.5)(57.0,23.5)(57,27.0)}  %step 0->1
\put(0,0){\color{yellow}\linethickness{0.1pt} \polygon(68.6, 27.1)(68.6, 24.7)(71, 24.7)(71, 27.1)}

\put(0,0){\color{blue}\linethickness{0.1pt} \polygon(39.6, 48.2)(39.6, 0.0)(68.1, 0.0)(68.1, 48.2)}  %step 0->1

\end{Overpic}
\caption{\textbf{Comparison of rollout frames in OBJ3D} with high dpi. RSM generates frames with precise dynamics and maintains visual quality, even during complex actions in steps 20 to 40. In contrast, the baselines produce ones with artifacts (yellow boxes) and inaccurate dynamics (red boxes).}
\label{fig:fullsteps_main_new}
% \vspace{-5mm}
\end{figure}




==> tables/ood_main.tex <==
% \begin{table*}[t]
% \caption{Comparison between the proposed RSM and the baselines in OOD setting. The number denotes ranking scores in percentage (\%) for multi-step prediction into the future in latent space. The reported scores are mean and Standard Error over 30 runs. The higher results indicate the better prediction. The best scores are \textbf{bolded}.}
% \label{table:ood_result}
% \begin{center}
% \begin{tabular}{clcccccc}
% \hline & \\[-1.0em]
% & & \multicolumn{2}{c}{\textit{1 step}} & \multicolumn{2}{c}{\textit{5 steps}} & \multicolumn{2}{c}{\textit{10 steps}} \\ \hline & \\[-1.0em]
% & \textit{\textbf{}} & \textbf{H@1} & \textbf{MRR} & \textbf{H@1} & \textbf{MRR} & \textbf{H@1} & \textbf{MRR} \\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Shapes}}} 
% & C-SWM & 93.0\textcolor{lightgray}{±0.6} & 95.9\textcolor{lightgray}{±0.5} & 81.3\textcolor{lightgray}{±0.7} & 86.5\textcolor{lightgray}{±0.7} & 72.1\textcolor{lightgray}{±0.8} & 78.6\textcolor{lightgray}{±0.7}\\
% & MBRL & 95.9\textcolor{lightgray}{±0.2} & 97.9\textcolor{lightgray}{±0.1} & 85.3\textcolor{lightgray}{±0.3} & 90.6\textcolor{lightgray}{±0.3} & 69.7\textcolor{lightgray}{±0.8} & 78.5\textcolor{lightgray}{±0.6}\\
% & NPS & 95.2\textcolor{lightgray}{±0.2} & 97.4\textcolor{lightgray}{±0.2} & 81.7\textcolor{lightgray}{±0.6} & 87.8\textcolor{lightgray}{±0.5} & 65.5\textcolor{lightgray}{±0.5} & 74.7\textcolor{lightgray}{±0.5}\\
% & RSM  (Ours) & \textbf{96.8}\textcolor{lightgray}{±0.0} & \textbf{98.4}\textcolor{lightgray}{±0.0} & \textbf{91.1}\textcolor{lightgray}{±0.2} & \textbf{94.6}\textcolor{lightgray}{±0.1} & \textbf{80.9}\textcolor{lightgray}{±0.3} & \textbf{87.2}\textcolor{lightgray}{±0.2}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Cubes}}} 
% & C-SWM & 78.1\textcolor{lightgray}{±5.5} & 85.7\textcolor{lightgray}{±4.3} & 52.7\textcolor{lightgray}{±8.7} & 63.8\textcolor{lightgray}{±7.7} & 40.6\textcolor{lightgray}{±8.3} & 51.7\textcolor{lightgray}{±8.0}\\
% & MBRL & 95.2\textcolor{lightgray}{±0.3} & 97.5\textcolor{lightgray}{±0.2} & 85.6\textcolor{lightgray}{±1.3} & 90.9\textcolor{lightgray}{±0.8} & 71.3\textcolor{lightgray}{±1.9} & 80.0\textcolor{lightgray}{±1.4}\\
% & NPS & 94.4\textcolor{lightgray}{±0.7} & 96.9\textcolor{lightgray}{±0.6} & 75.4\textcolor{lightgray}{±4.2} & 80.3\textcolor{lightgray}{±3.4} & 63.2\textcolor{lightgray}{±5.4} & 70.5\textcolor{lightgray}{±4.9}\\
% & RSM  (Ours) & \textbf{97.5}\textcolor{lightgray}{±0.2} & \textbf{99.7}\textcolor{lightgray}{±0.1} & \textbf{89.6}\textcolor{lightgray}{±0.9} & \textbf{94.5}\textcolor{lightgray}{±0.6} & \textbf{77.5}\textcolor{lightgray}{±1.5} & \textbf{86.3}\textcolor{lightgray}{±1.1}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Breakout}}} 
% & C-SWM & 27.0\textcolor{lightgray}{±3.8} & 44.5\textcolor{lightgray}{±3.9} & 5.4\textcolor{lightgray}{±1.0} & 16.4\textcolor{lightgray}{±1.4} & 2.8\textcolor{lightgray}{±0.7} & 10.3\textcolor{lightgray}{±1.2}\\
% & MBRL & 30.7\textcolor{lightgray}{±4.0} & 48.3\textcolor{lightgray}{±3.2} & 4.6\textcolor{lightgray}{±0.3} & 13.9\textcolor{lightgray}{±0.5} & 2.1\textcolor{lightgray}{±0.3} & 9.5\textcolor{lightgray}{±0.3}\\
% & NPS & 28.1\textcolor{lightgray}{±1.5} & 46.2\textcolor{lightgray}{±0.5} & 4.9\textcolor{lightgray}{±2.0} & 11.5\textcolor{lightgray}{±1.0} & 3.9\textcolor{lightgray}{±1.0} & 10.2\textcolor{lightgray}{±1.2}\\
% & RSM (Ours) & \textbf{39.8}\textcolor{lightgray}{±0.1} & \textbf{56.3}\textcolor{lightgray}{±0.7} & \textbf{19.1}\textcolor{lightgray}{±0.4} & \textbf{32.7}\textcolor{lightgray}{±1.0} & \textbf{10.1}\textcolor{lightgray}{±1.2} & \textbf{19.3}\textcolor{lightgray}{±0.8}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Pong}}} 
% & C-SWM & 10.8\textcolor{lightgray}{±2.4} & 25.0\textcolor{lightgray}{±3.9} & 2.1\textcolor{lightgray}{±0.5} & 9.3\textcolor{lightgray}{±0.8} & 2.0\textcolor{lightgray}{±0.4} & 8.6\textcolor{lightgray}{±0.7}\\
% & MBRL & 15.9\textcolor{lightgray}{±2.0} & 34.1\textcolor{lightgray}{±2.5} & 2.5\textcolor{lightgray}{±0.3} & 9.8\textcolor{lightgray}{±0.6} & 1.7\textcolor{lightgray}{±0.3} & 7.4\textcolor{lightgray}{±0.5}\\
% & NPS & 14.6\textcolor{lightgray}{±3.2} & 32.1\textcolor{lightgray}{±4.4} & 2.0\textcolor{lightgray}{±0.4} & 9.7\textcolor{lightgray}{±1.1} & 0.8\textcolor{lightgray}{±0.4} & 6.4\textcolor{lightgray}{±0.4}\\
% & RSM (Ours) & \textbf{41.6}\textcolor{lightgray}{±0.8} & \textbf{57.1}\textcolor{lightgray}{±1.6} & \textbf{24.8}\textcolor{lightgray}{±1.6} & \textbf{36.9}\textcolor{lightgray}{±1.9} & \textbf{18.6}\textcolor{lightgray}{±2.1} & \textbf{25.2}\textcolor{lightgray}{±2.2}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Balls}}} 
% & C-SWM & 76.8\textcolor{lightgray}{±5.5} & 86.0\textcolor{lightgray}{±3.8} & 11.6\textcolor{lightgray}{±2.8} & 23.5\textcolor{lightgray}{±4.6} & 2.6\textcolor{lightgray}{±0.8} & 8.2\textcolor{lightgray}{±1.9}\\
% & MBRL & 74.8\textcolor{lightgray}{±4.8} & 85.1\textcolor{lightgray}{±3.1} & 9.9\textcolor{lightgray}{±2.5} & 21.3\textcolor{lightgray}{±3.9} & 2.6\textcolor{lightgray}{±0.8} & 7.7\textcolor{lightgray}{±1.6}\\
% & NPS & 78.2\textcolor{lightgray}{±0.4} & 87.6\textcolor{lightgray}{±0.1} & 11.1\textcolor{lightgray}{±3.7} & 29.1\textcolor{lightgray}{±4.3} & 9.3\textcolor{lightgray}{±3.8} & 12.7\textcolor{lightgray}{±4.7}\\
% & RSM  (Ours) & \textbf{84.3}\textcolor{lightgray}{±1.9} & \textbf{91.4}\textcolor{lightgray}{±1.1} & \textbf{28.3}\textcolor{lightgray}{±4.2} & \textbf{43.4}\textcolor{lightgray}{±4.8} & \textbf{19.6}\textcolor{lightgray}{±2.4} & \textbf{27.1}\textcolor{lightgray}{±3.3}\\
% \hline
% \end{tabular}
% \end{center}
% \end{table*}


\begin{table*}[!t]
\caption{\textbf{Comparison of the prediction in latent space} between the proposed RSM and the baselines in both iid and OOD test sets. 
The mean and standard error of ranks over 30 seeds are reported.
Larger scores indicate better predictions. The best scores are in \textbf{bold}, with RSM winning much more often than any of the baselines, and always winning OOD.}
\label{table:ab_result}
\begin{center}
\small
\begin{tabular}{ll|ccc|ccc}
\hline & \\[-10pt]
& & \multicolumn{3}{c|}{\textbf{iid}} & \multicolumn{3}{c}{\textbf{OOD}} \\ \hline & \\[-1.0em]
& \textit{\textbf{}} & \textit{1 step} & \textit{5 steps} & \textit{10 steps} & \textit{1 step} & \textit{5 steps} & \textit{10 steps} \\
\hline & \\[-10pt] 
\multirow{4}{9pt}{\rotatebox{90}{\textbf{Shapes}}} 
& C-SWM & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{100.0}\textcolor{lightgray}{±0.0} & 93.0\textcolor{lightgray}{±0.6} & 81.3\textcolor{lightgray}{±0.7} & 72.1\textcolor{lightgray}{±0.8} \\
& MBRL & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.8\textcolor{lightgray}{±0.0} & 98.0\textcolor{lightgray}{±0.1} & 95.9\textcolor{lightgray}{±0.2} & 85.3\textcolor{lightgray}{±0.3} & 69.7\textcolor{lightgray}{±0.8}\\
& NPS & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.7\textcolor{lightgray}{±0.1} & 97.0\textcolor{lightgray}{±0.3} & 95.2\textcolor{lightgray}{±0.2} & 81.7\textcolor{lightgray}{±0.6} & 65.5\textcolor{lightgray}{±0.5}\\
& RSM (Ours) & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.9\textcolor{lightgray}{±0.0} & 97.9\textcolor{lightgray}{±0.1} & \textbf{96.8}\textcolor{lightgray}{±0.0} & \textbf{91.1}\textcolor{lightgray}{±0.2} & \textbf{80.9}\textcolor{lightgray}{±0.3}\\
\hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Cubes}}} 
& C-SWM & \textbf{100.0}\textcolor{lightgray}{±0.2} & \textbf{99.6}\textcolor{lightgray}{±0.0} & \textbf{98.2}\textcolor{lightgray}{±0.5} & 78.1\textcolor{lightgray}{±5.5} & 52.7\textcolor{lightgray}{±8.7} & 40.6\textcolor{lightgray}{±8.3}\\
& MBRL & 99.8\textcolor{lightgray}{±0.1} & 99.1\textcolor{lightgray}{±0.2} & 96.5\textcolor{lightgray}{±0.4} & 95.2\textcolor{lightgray}{±0.3} & 85.6\textcolor{lightgray}{±1.3} & 71.3\textcolor{lightgray}{±1.9}\\
& NPS & 99.8\textcolor{lightgray}{±0.2} & 99.1\textcolor{lightgray}{±0.6} & 96.6\textcolor{lightgray}{±1.6} & 94.4\textcolor{lightgray}{±0.7} & 75.4\textcolor{lightgray}{±4.2} & 63.2\textcolor{lightgray}{±5.4}\\
& RSM (Ours) & 99.8\textcolor{lightgray}{±0.0} & 99.2\textcolor{lightgray}{±0.6} & 93.9\textcolor{lightgray}{±1.5} & \textbf{97.5}\textcolor{lightgray}{±0.2} & \textbf{89.6}\textcolor{lightgray}{±0.9} & \textbf{77.5}\textcolor{lightgray}{±1.5}\\
% \hline  \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Breakout}}}
% & C-SWM & 65.6\textcolor{lightgray}{±4.1} & 36.7\textcolor{lightgray}{±3.7} & 21.8\textcolor{lightgray}{±2.2} & 27.0\textcolor{lightgray}{±3.8} & 5.4\textcolor{lightgray}{±1.0} & 2.8\textcolor{lightgray}{±0.7}\\
% & MBRL & 64.7\textcolor{lightgray}{±1.2} & 37.4\textcolor{lightgray}{±1.8} & 14.9\textcolor{lightgray}{±2.1} & 30.7\textcolor{lightgray}{±4.0} & 4.6\textcolor{lightgray}{±0.3} & 2.1\textcolor{lightgray}{±0.3}\\
% & NPS & 68.0\textcolor{lightgray}{±0.3} & 44.5\textcolor{lightgray}{±1.1} & \textbf{27.2}\textcolor{lightgray}{±1.5} & 28.1\textcolor{lightgray}{±1.5} & 4.9\textcolor{lightgray}{±2.0} & 3.9\textcolor{lightgray}{±1.0}\\
% & RSM (Ours) & \textbf{73.3}\textcolor{lightgray}{±1.0} & \textbf{46.6}\textcolor{lightgray}{±1.7} & \textbf{27.2}\textcolor{lightgray}{±2.0} & \textbf{39.8}\textcolor{lightgray}{±0.1} & \textbf{19.1}\textcolor{lightgray}{±0.4} & \textbf{10.1}\textcolor{lightgray}{±1.2}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Pong}}}
% & C-SWM & 44.2\textcolor{lightgray}{±4.9} & 21.4\textcolor{lightgray}{±1.9} & 15.2\textcolor{lightgray}{±1.7} & 10.8\textcolor{lightgray}{±2.4} & 2.1\textcolor{lightgray}{±0.5} & 2.0\textcolor{lightgray}{±0.4}\\
% & MBRL & 50.3\textcolor{lightgray}{±2.0} & 23.9\textcolor{lightgray}{±1.5} & 16.8\textcolor{lightgray}{±2.1} & 15.9\textcolor{lightgray}{±2.0} & 2.5\textcolor{lightgray}{±0.3} & 1.7\textcolor{lightgray}{±0.3}\\
% & NPS & 52.0\textcolor{lightgray}{±5.0} & 24.2\textcolor{lightgray}{±1.6} & 15.4\textcolor{lightgray}{±2.2} & 14.6\textcolor{lightgray}{±3.2} & 2.0\textcolor{lightgray}{±0.4} & 0.8\textcolor{lightgray}{±0.4}\\
% & RSM (Ours) & \textbf{53.9}\textcolor{lightgray}{±1.5} & \textbf{30.6}\textcolor{lightgray}{±1.0} & \textbf{23.5}\textcolor{lightgray}{±0.7} & \textbf{41.6}\textcolor{lightgray}{±0.8} & \textbf{24.8}\textcolor{lightgray}{±1.6} & \textbf{18.6}\textcolor{lightgray}{±2.1}\\
% \hline & \\[-10pt] \multirow{4}{9pt}{\rotatebox{90}{\textbf{Balls}}} 
% & C-SWM & 99.7\textcolor{lightgray}{±0.1} & 86.6\textcolor{lightgray}{±4.9} & 64.9\textcolor{lightgray}{±8.8} & 76.8\textcolor{lightgray}{±5.5} & 11.6\textcolor{lightgray}{±2.8} & 2.6\textcolor{lightgray}{±0.8}\\
% & MBRL & 99.8\textcolor{lightgray}{±0.1} & 89.7\textcolor{lightgray}{±4.5} & 68.1\textcolor{lightgray}{±6.0} & 74.8\textcolor{lightgray}{±4.8} & 9.9\textcolor{lightgray}{±2.5} & 2.6\textcolor{lightgray}{±0.8}\\
% & NPS & \textbf{100.0}\textcolor{lightgray}{±0.0} & 89.5\textcolor{lightgray}{±1.9} & \textbf{73.2}\textcolor{lightgray}{±3.3} & 78.2\textcolor{lightgray}{±0.4} & 11.1\textcolor{lightgray}{±3.7} & 9.3\textcolor{lightgray}{±3.8}\\
% & RSM (Ours) & 99.8\textcolor{lightgray}{±0.0} & \textbf{92.9}\textcolor{lightgray}{±1.8} & 72.6\textcolor{lightgray}{±4.5} & \textbf{84.3}\textcolor{lightgray}{±1.9} & \textbf{28.3}\textcolor{lightgray}{±4.2} & \textbf{19.6}\textcolor{lightgray}{±2.4}\\
\hline \\
\end{tabular}
\end{center}
\label{tab:merge_table}
\end{table*}





==> tables/rebuttal_sec1.tex <==
\begin{figure}[h]
\centering
% \small
\begin{Overpic}[abs,unit=1mm,grid=false,tics=3]{%
\begin{tabular}{*{14}{@{\hspace{-1px}}c}}
   & $t=0$  & 2 & 4 &  6 & 8 & 10 & 12 & 14 & 16 & 18 & 20 & 22 \\
    \textbf{Gold} & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_0_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_2_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_4_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_6_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_8_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_10_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_12_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_14_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_16_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_18_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_20_0.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_22_0.pdf}} 
     \\ & \\ & \\ \\[-12.5pt]
    \textbf{RSM} &   \multicolumn{5}{c}{10 burn-in frames}
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_10_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_12_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_14_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_16_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_18_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_20_1.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec1/video_53_22_1.pdf}}  
     \\ & \\ & \\ \\[-2.5pt]
     % & Step=0 & Slot 1& Slot 2 & Slot 3 & Slot 4 & Slot 5 & Slot 6 & Slot 7 & Slot 8   \\
  % \textbf{SlotFormer}  &  - & - & - & - & -
  %    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_pred_step08.pdf}} 
  %    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_pred_step09.pdf}} 
  %    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_pred_step10.pdf}} 
  %    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_pred_step11.pdf}} 
  %    & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_pred_step12.pdf}} 
  %    \\ & \\ & \\ \\[-4.7pt]
  \end{tabular}}%
% \put(1,6){\color{yellow}\vector(4,-6){2.3}}
% % \put(0,0){\color{red}\linethickness{1pt} \polygon(83, 21.75)(83, 19)(88.5,19)(88.5,21.75)}  %step 0->1
% % \put(0,0){\color{yellow}\linethickness{1pt} \polygon(35.4, 21)(35.4, 16.7)(42, 16.7)(42, 21)}  %step 0->1

\end{Overpic}
\vspace{-5mm}
\caption{\textbf{ Experiment Results on a Highly Realistic Dataset - MOVi-C}. RSM generates prospective rollout frames that capture dynamic object behaviors, as demonstrated by the white can's rightward movement and the lion toy's downward motion. Despite certain constraints in the visual of current predicted next frames, these initial results, with the ability to respond to objects' dynamics, facilitate further training and fine-tuning both object-centric and RSM models to tackle this family of  realistic scene datasets, and real scene data. }
\label{fig:fullsteps_main_}% 
\end{figure}












==> tables/rebuttal_sec2.tex <==
\begin{figure}[h]
\centering
\small
\begin{Overpic}[abs,unit=1mm,grid=false,tics=3]{%
\begin{tabular}{*{12}{@{\hspace{1px}}c}}
    Rollout & Pred & Slot 1 & Slot 2 & Slot 4 & Slot 6 & & Pred & Slot 1 & Slot 2 & Slot 3 & Slot 4\\
      
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step12_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step12_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step12_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step12_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step12_7.png}} 
     &
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step42_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step42_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step42_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step42_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step42_5.png}} 
     \\ 
    $t = 12$ & & & & & & $t = 42$\\
     & \\ \\[-14pt]
     Mechanism & 
     & Idle & M.Fast & Idle & Idle 
     & \quad Mechanism  
     & & M.Spin & M.Slow & M.Fast & M.Spin
     \\ \\[-12.0 pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step14_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step14_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step14_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step14_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step14_7.png}} 
     &  
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step44_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step44_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step44_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step44_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step44_5.png}} 
      \\ 
    $t=14$ & & & & & & $t=44$\\
     & \\ \\[-14pt]
    Mechanism & 
      & Collide & Collide & Idle & Idle & \quad Mechanism & & M.Spin & M.Slow & M.Fast & M.Spin 
     \\ \\[-12 pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step20_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step20_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step20_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step20_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step20_7.png}} 
     &  
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step46_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step46_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step46_3.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step46_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_ob/ob_step46_5.png}} 
      \\
     $t=20$ & & & & & & $t=46$\\  \\ \\[-14pt]

     Mechanism & & M.Fast & M.Fast & Collide & Idle
     & \quad Mechanism
     & & M.Spin & M.Slow & M.Fast & M.Spin 
     % & \\ \\[-12.2pt]
\end{tabular}}%

% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(65.5, 47.6)(65.5, 35.6)(75, 35.6)(75, 47.6)}  %step 0->1
% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(85.0, 47.6)(85.0, 35.6)(94.5, 35.6)(94.5, 47.6)}  %step 0->1

% \put(0,0){\color{green}\linethickness{0.3pt} \polygon(65.5, 11.8)(65.5, 0.0)(75, 0.0)(75, 11.8)}  %step 0->1
% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(85.0, 11.8)(85.0, 0.0)(94.5, 0.0)(94.5, 11.8)}  %step 0->1
\end{Overpic}
\caption{\textbf{Mechanism assignment in OBJ3D} on 4 over 6 slots. 
The  mechanisms can be inferred as follow: \textbf{Idle}, \textbf{M}oving \textbf{fast} (M.Fast), \textbf{M}oving and \textbf{spin}ning (M.Spin), \textbf{Collide},  and \textbf{M}oving \textbf{slow} (M.Slow). The spinning movement is observed better in the video format.
}
\label{fig:4steps_attn}
% \vspace{-5mm}
\end{figure}



\begin{figure}[h]
\centering
\small
\begin{Overpic}[abs,unit=1mm,grid=false,tics=3]{%
\begin{tabular}{*{12}{@{\hspace{-1px}}c}}
      Rollout & Pred & Slot 2 & Slot 4 & Slot 6 & Slot 7 & & Pred & Slot 1 & Slot 2 & Slot 5 & Slot 6 \\
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step23_0.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step23_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step23_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step23_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step23_7.png}} 
     &
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step14_0.png}} 
     % & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{rsm2/rollout_vis/mech_vis/PHYRE/pred_slots/PHYRE_slotformer_dp5_slot0005_step06.pdf}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step14_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step14_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step14_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step14_6.png}} 
     \\ 
    $t = 23$ & & & & & & $t = 14$\\
     & \\ \\[-14pt]
     Mechanism & 
     & M.Slow & M.Fast & M.Fast & Idle 
     & \quad Mechanism  
     & & Idle & Idle & M.Fast & Idle
     \\ \\[-12.2pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step27_0.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step27_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step27_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step27_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step27_7.png}} 
     &  
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step15_0.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step15_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step15_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step15_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step15_6.png}} 
      \\ 
    $t=27$ & & & & & & $t=15$\\
     & \\ \\[-14pt]
    Mechanism & 
      & M.Slow & Collide & Collide & Idle & \quad Mechanism & & Idle & Idle & Collide & Collide
     \\ \\[-12.2pt]
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step35_0.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step35_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step35_4.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step35_6.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id1_step35_7.png}} 
     &  
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step16_0.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step16_1.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step16_2.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step16_5.png}} 
     & \multirow{3}{0.04\textheight}{\includegraphics[height=0.04\textheight]{tables/rebuttal/sec2_clevrer/id2_step16_6.png}} 
      \\
     $t=35$ & & & & & & $t=16$\\  \\ \\[-14pt]
     Mechanism & & M.Slow & M.Fast & M.Spin & Idle
     & \quad Mechanism
     & & Idle & Idle & M.Fast & M.Fast 
     % & \\ \\[-12.2pt]
  \end{tabular}}%
% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(65.5, 47.6)(65.5, 35.6)(75, 35.6)(75, 47.6)}  %step 0->1
% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(85.0, 47.6)(85.0, 35.6)(94.5, 35.6)(94.5, 47.6)}  %step 0->1
% \put(0,0){\color{green}\linethickness{0.3pt} \polygon(65.5, 11.8)(65.5, 0.0)(75, 0.0)(75, 11.8)}  %step 0->1
% \put(0,0){\color{blue}\linethickness{0.3pt} \polygon(85.0, 11.8)(85.0, 0.0)(94.5, 0.0)(94.5, 11.8)}  %step 0->1
\end{Overpic}
\caption{\textbf{Mechanisms assignment in CLEVRER} on 4 over 7 slots. 
The  mechanisms can be inferred as follow:   \textbf{Idle},  \textbf{Collide},  \textbf{M}oving \textbf{slow}  (M.slow),  \textbf{M}oving \textbf{fast}  (M.Fast), and \textbf{M}oving and \textbf{spin}ning (M.Spin). The spinning movement is observed better in the video format.
}
\label{fig:4steps_attn}
% \vspace{-5mm}
\end{figure}




==> tables/usage_ctx.tex <==
\begin{table*}[!t]
\caption{\textbf{Comparison on ablation studies}. 
The reported scores are mean and standard error over 30 seeds of ranking scores for multi-step prediction into the future.
The higher scores indicate a better prediction. The best scores are \textbf{bolded}.}
\label{table:ab_result}
\begin{center}
\begin{tabular}{ll|ccc|ccc}
\hline & \\[-10pt]
& & \multicolumn{3}{c|}{\textbf{IID}} & \multicolumn{3}{c}{\textbf{OOD}} \\ \hline & \\[-1.0em]
& \textit{\textbf{}} & \textit{1 step} & \textit{5 steps} & \textit{10 steps} & \textit{1 step} & \textit{5 steps} & \textit{10 steps} \\
\hline & \\[-10pt] 
\multirow{6}{9pt}{\rotatebox{90}{\textbf{Shapes}}} 
& RSM (Ours) & \textbf{100.0}\textcolor{lightgray}{±0.0} &  \textbf{99.9}\textcolor{lightgray}{±0.0} &  \textbf{97.9}\textcolor{lightgray}{±0.1} & \textbf{96.8}\textcolor{lightgray}{±0.0} & \textbf{91.1}\textcolor{lightgray}{±0.2} & \textbf{80.9}\textcolor{lightgray}{±0.3} \\
& RSM ab 01 & \textbf{100.0}\textcolor{lightgray}{±0.0} & 99.0\textcolor{lightgray}{±0.4} & 94.7\textcolor{lightgray}{±1.3} & 96.7\textcolor{lightgray}{±0.1} &  86.4\textcolor{lightgray}{±1.4} & 71.8\textcolor{lightgray}{±2.9} \\
& RSM ab 10 & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{99.9}\textcolor{lightgray}{±0.0} & 97.4\textcolor{lightgray}{±0.1} & 96.9\textcolor{lightgray}{±0.0} & 89.9\textcolor{lightgray}{±0.3} & 79.6\textcolor{lightgray}{±0.6}\\
& RSM ab 00 & \textbf{100.0}\textcolor{lightgray}{±0.0} & 98.8\textcolor{lightgray}{±0.0} & 90.5\textcolor{lightgray}{±0.1} & 96.8\textcolor{lightgray}{±0.0} & 77.7\textcolor{lightgray}{±0.4} & 52.4\textcolor{lightgray}{±0.8} \\
& RSM ab par & \textbf{100.0}\textcolor{lightgray}{±0.0} & \textbf{99.9}\textcolor{lightgray}{±0.0} & 97.5\textcolor{lightgray}{±0.1} & 96.7\textcolor{lightgray}{±0.1} & 90.2\textcolor{lightgray}{±0.4} & 80.2\textcolor{lightgray}{±0.5} \\
& MLP-CCI & \textbf{100.0}\textcolor{lightgray}{±0.0} & 94.8\textcolor{lightgray}{±0.0} & 89.8\textcolor{lightgray}{±0.1} & 95.6\textcolor{lightgray}{±0.2} & 86.1\textcolor{lightgray}{±0.4} & 70.3\textcolor{lightgray}{±1.0} \\
\hline & \\[-10pt] \multirow{6}{9pt}{\rotatebox{90}{\textbf{Cubes}}} 
& RSM (Ours) & 99.8\textcolor{lightgray}{±0.0} & \textbf{99.2}\textcolor{lightgray}{±0.6} & \textbf{93.9}\textcolor{lightgray}{±1.5}  & \textbf{97.5}\textcolor{lightgray}{±0.2} & \textbf{89.6}\textcolor{lightgray}{±0.9} & \textbf{77.5}\textcolor{lightgray}{±1.5} \\
& RSM ab 01 & 99.8\textcolor{lightgray}{±0.0} & 94.7\textcolor{lightgray}{±0.8} & 86.0\textcolor{lightgray}{±2.1} & 94.6\textcolor{lightgray}{±0.3} & 80.9\textcolor{lightgray}{±1.4} & 65.2\textcolor{lightgray}{±1.8} \\
& RSM ab 10 & \textbf{100.0}\textcolor{lightgray}{±0.0} & 98.0\textcolor{lightgray}{±0.7} & 93.8\textcolor{lightgray}{±1.7} & 96.0\textcolor{lightgray}{±0.1} & 84.4\textcolor{lightgray}{±0.6} & 69.0\textcolor{lightgray}{±0.9} \\
& RSM ab 00 & \textbf{100.0}\textcolor{lightgray}{±0.0} & 91.9\textcolor{lightgray}{±0.7} & 82.5\textcolor{lightgray}{±1.6} & 94.4\textcolor{lightgray}{±0.5} & 72.6\textcolor{lightgray}{±1.3} & 48.0\textcolor{lightgray}{±2.8} \\ 
& RSM ab par &  99.8\textcolor{lightgray}{±0.0} & 95.5\textcolor{lightgray}{±0.6} & 87.4\textcolor{lightgray}{±1.3} & 94.8\textcolor{lightgray}{±0.5} & 80.6\textcolor{lightgray}{±1.5} & 65.7\textcolor{lightgray}{±1.9} \\
& MLP-CCI & 99.7\textcolor{lightgray}{±0.0} & 87.8\textcolor{lightgray}{±0.3} & 81.7\textcolor{lightgray}{±0.6} & 93.6\textcolor{lightgray}{±0.3} & 80.6\textcolor{lightgray}{±1.0} & 60.4\textcolor{lightgray}{±1.5} \\
\hline & \\[-10pt] \multirow{6}{9pt}{\rotatebox{90}{\textbf{Breakout}}} 
& RSM (Ours) & 73.3\textcolor{lightgray}{±1.0} & 46.6\textcolor{lightgray}{±1.7} & 27.2\textcolor{lightgray}{±2.0} & \textbf{39.8}\textcolor{lightgray}{±0.1} & \textbf{19.1}\textcolor{lightgray}{±0.4} & \textbf{10.1}\textcolor{lightgray}{±1.2} \\
& RSM ab 01 & 69.3\textcolor{lightgray}{±2.6} & 39.8\textcolor{lightgray}{±3.0} & 23.4\textcolor{lightgray}{±3.1} & 22.3\textcolor{lightgray}{±2.1} & 4.0\textcolor{lightgray}{±0.7} & 2.1\textcolor{lightgray}{±0.7}\\
& RSM ab 10 & \textbf{74.5}\textcolor{lightgray}{±1.4} & \textbf{54.5}\textcolor{lightgray}{±2.8} & \textbf{32.9}\textcolor{lightgray}{±2.3} & 22.8\textcolor{lightgray}{±2.2} & 4.4\textcolor{lightgray}{±0.9} & 2.2\textcolor{lightgray}{±0.5} \\
& RSM ab 00 & 46.3\textcolor{lightgray}{±4.1} & 25.3\textcolor{lightgray}{±2.8} & 18.8\textcolor{lightgray}{±2.1} & 20.0\textcolor{lightgray}{±1.8} & 5.1\textcolor{lightgray}{±0.6} & 2.6\textcolor{lightgray}{±0.5}\\
& RSM ab par & 72.5\textcolor{lightgray}{±0.9} & 41.6\textcolor{lightgray}{±1.7} & 22.4\textcolor{lightgray}{±1.0} & 22.1\textcolor{lightgray}{±1.4} & 5.5\textcolor{lightgray}{±0.6} & 2.5\textcolor{lightgray}{±0.6} \\
& MLP-CCI & 70.1\textcolor{lightgray}{±1.5} & 39.3\textcolor{lightgray}{±3.0} & 23.9\textcolor{lightgray}{±2.6} & 29.2\textcolor{lightgray}{±4.0} & 6.3\textcolor{lightgray}{±0.5} & 3.2\textcolor{lightgray}{±0.7} \\
\hline & \\[-10pt] \multirow{6}{9pt}{\rotatebox{90}{\textbf{Pong}}} 
& RSM (Ours) & \textbf{53.9}\textcolor{lightgray}{±1.5} & \textbf{30.6}\textcolor{lightgray}{±1.0} & \textbf{23.5}\textcolor{lightgray}{±0.7} & \textbf{41.6}\textcolor{lightgray}{±0.8} & \textbf{24.8}\textcolor{lightgray}{±1.6} & \textbf{18.6}\textcolor{lightgray}{±2.1} \\
& RSM ab 01 & 43.5\textcolor{lightgray}{±3.1} & 21.3\textcolor{lightgray}{±1.1} & 15.0\textcolor{lightgray}{±1.4} & 15.2\textcolor{lightgray}{±2.5} & 2.5\textcolor{lightgray}{±0.3} & 2.2\textcolor{lightgray}{±0.3} \\
& RSM ab 10 & 44.9\textcolor{lightgray}{±4.3} & 24.3\textcolor{lightgray}{±2.2} & 20.7\textcolor{lightgray}{±2.5} & 26.7\textcolor{lightgray}{±3.5} & 13.1\textcolor{lightgray}{±0.2} & 11.8\textcolor{lightgray}{±0.4} \\
& RSM ab 00 & 41.8\textcolor{lightgray}{±5.7} & 20.5\textcolor{lightgray}{±4.9} & 18.7\textcolor{lightgray}{±4.1} & 9.7\textcolor{lightgray}{±4.3} & 2.7\textcolor{lightgray}{±0.5} & 1.3\textcolor{lightgray}{±0.3} \\
& RSM ab par & 50.4\textcolor{lightgray}{±3.4} & 24.3\textcolor{lightgray}{±1.6} & 20.9\textcolor{lightgray}{±1.2} & 18.1\textcolor{lightgray}{±2.7} & 2.1\textcolor{lightgray}{±0.4} & 1.9\textcolor{lightgray}{±0.5}\\
& MLP-CCI & 45.9\textcolor{lightgray}{±3.3} & 24.1\textcolor{lightgray}{±2.5} & 18.1\textcolor{lightgray}{±2.3} & 15.2\textcolor{lightgray}{±2.8} & 3.1\textcolor{lightgray}{±0.5} & 1.9\textcolor{lightgray}{±0.5} \\
\hline & \\[-10pt] \multirow{6}{9pt}{\rotatebox{90}{\textbf{Balls}}} 
& RSM (Ours) & \textbf{99.8}\textcolor{lightgray}{±0.0} & \textbf{92.9}\textcolor{lightgray}{±1.8} & 72.6\textcolor{lightgray}{±4.5} & \textbf{84.3}\textcolor{lightgray}{±1.9} & \textbf{28.3}\textcolor{lightgray}{±4.2} & \textbf{19.6}\textcolor{lightgray}{±2.4} \\
& RSM ab 01 & 99.6\textcolor{lightgray}{±0.1} & 89.2\textcolor{lightgray}{±3.7} & 68.8\textcolor{lightgray}{±5.9} & 81.2\textcolor{lightgray}{±1.4} & 12.1\textcolor{lightgray}{±0.9} & 4.1\textcolor{lightgray}{±0.5} \\
& RSM ab 10 & 99.7\textcolor{lightgray}{±0.0} & 93.2\textcolor{lightgray}{±1.1} & 68.8\textcolor{lightgray}{±2.4} & 83.2\textcolor{lightgray}{±1.4} & 12.7\textcolor{lightgray}{±1.8} & 5.1\textcolor{lightgray}{±0.8} \\
& RSM ab 00 & \textbf{99.8}\textcolor{lightgray}{±0.0} & 92.8\textcolor{lightgray}{±0.9} & 67.9\textcolor{lightgray}{±2.3} & 82.9\textcolor{lightgray}{±1.5} & 13.1\textcolor{lightgray}{±1.8} & 4.4\textcolor{lightgray}{±0.8} \\
& RSM ab par & 99.7\textcolor{lightgray}{±0.0} & 90.7\textcolor{lightgray}{±2.7} & 69.8\textcolor{lightgray}{±5.6} & 80.3\textcolor{lightgray}{±2.2} & 11.9\textcolor{lightgray}{±3.4} & 4.5\textcolor{lightgray}{±1.6} \\
& MLP-CCI & 99.8\textcolor{lightgray}{±0.0} & 90.3\textcolor{lightgray}{±1.2} & 71.2\textcolor{lightgray}{±3.3} & 84.6\textcolor{lightgray}{±3.4} & 21.3\textcolor{lightgray}{±4.7} & 7.0\textcolor{lightgray}{±2.5} \\
\hline \\
\end{tabular}
\end{center}
\label{ta:ab_full}
\end{table*}


